Pixels or Code? Benchmarking Instruction-Guided Visual Artifact Operation

Visual artifacts such as charts, technical diagrams, webpages, and document pages underpin scientific, commercial, and engineering workflows. Editing these artifacts requires direct modification, dependency-aware updates, preservation of unaffected content, and compliance with domain constraints. We define this capability as Visual Artifact Operation (VAO). Prior benchmarks test parts of this problem, including cascading updates in charts. We study direct edits, dependent updates, and preservation across visual domains and pixel, code, and agent paradigms under one image-only protocol. We introduce Visual Artifact Operation Bench (VAO-Bench), comprising 1,573 manually screened tasks across nine artifact categories and three difficulty levels. VAO-Bench uses executable artifacts and deterministic rendering to trace reference transformations and annotate direct edits, dependent updates, and preservation constraints. All systems receive the same source image and instruction; we evaluate pixel-space editors, code-generating multimodal systems, and tool-using agents on direct-edit accuracy, dependency-aware update, content preservation, domain validity, and visual quality. Experiments show that executable-code systems better support dependent updates, while pixel-space editors offer faster execution and strong visual quality. Explicitly stating dependencies improves both paradigms, identifying implicit-update inference as a central bottleneck. VAO-Bench provides a reproducible foundation for dependable visual artifact editing across generation paradigms.

==> prompts/construction.tex <==
\subsubsection{源产物生成}
\paragraph{step1\_source\_spec：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_03.txt}
\paragraph{step1\_source\_spec：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_27.txt}
\paragraph{step1\_source\_code：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_01.txt}
\paragraph{step1\_source\_code：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_25.txt}
\paragraph{step1\_source\_qa：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_09.txt}
\paragraph{step1\_source\_qa：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_33.txt}
\paragraph{step1\_source\_repair：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_02.txt}
\paragraph{step1\_source\_repair：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_26.txt}
\subsubsection{修改指令生成}
\paragraph{step2\_instruction\_candidates：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_04.txt}
\paragraph{step2\_instruction\_candidates：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_28.txt}
\paragraph{step2\_grounding\_check：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_10.txt}
\paragraph{step2\_grounding\_check：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_34.txt}
\paragraph{step2\_instruction\_repair：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_05.txt}
\paragraph{step2\_instruction\_repair：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_29.txt}
\subsubsection{目标产物生成}
\paragraph{step3\_operation\_plan：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_06.txt}
\paragraph{step3\_operation\_plan：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_30.txt}
\paragraph{step3\_target\_code：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_07.txt}
\paragraph{step3\_target\_code：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_31.txt}
\paragraph{step3\_source\_target\_compare：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_11.txt}
\paragraph{step3\_source\_target\_compare：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_35.txt}
\paragraph{step3\_target\_repair：通用模板。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_08.txt}
\paragraph{step3\_target\_repair：领域补充规则。}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_32.txt}


==> prompts/construction_en.tex <==
\subsubsection{Source Artifact Generation}
\paragraph{step1\_source\_spec:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_03.txt}
\paragraph{step1\_source\_spec:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_27.txt}
\paragraph{step1\_source\_code:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_01.txt}
\paragraph{step1\_source\_code:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_25.txt}
\paragraph{step1\_source\_qa:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_09.txt}
\paragraph{step1\_source\_qa:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_33.txt}
\paragraph{step1\_source\_repair:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_02.txt}
\paragraph{step1\_source\_repair:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_26.txt}
\subsubsection{Instruction Generation}
\paragraph{step2\_instruction\_candidates:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_04.txt}
\paragraph{step2\_instruction\_candidates:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_28.txt}
\paragraph{step2\_grounding\_check:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_10.txt}
\paragraph{step2\_grounding\_check:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_34.txt}
\paragraph{step2\_instruction\_repair:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_05.txt}
\paragraph{step2\_instruction\_repair:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_29.txt}
\subsubsection{Target Artifact Generation}
\paragraph{step3\_operation\_plan:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_06.txt}
\paragraph{step3\_operation\_plan:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_30.txt}
\paragraph{step3\_target\_code:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_07.txt}
\paragraph{step3\_target\_code:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_31.txt}
\paragraph{step3\_source\_target\_compare:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_11.txt}
\paragraph{step3\_source\_target\_compare:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_35.txt}
\paragraph{step3\_target\_repair:General Template.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_08.txt}
\paragraph{step3\_target\_repair:Category-Specific Rules.}
\VerbatimInput[fontsize=\tiny,baselinestretch=0.58,breaklines=true,breakanywhere=true,frame=single,framesep=3pt,rulecolor=promptline,backgroundcolor=promptbg]{prompts/prompt_compact_32.txt}


==> tables/compact_results_1.tex <==
\begingroup\fontsize{7.2}{8.4}\selectfont\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{@{}lrr*{10}{r}@{}}\toprule
 & & & \multicolumn{5}{c}{Auto-zero} & \multicolumn{5}{c}{Completed-only}\\
ID & 秒 & 完成率 & Dir. & Der. & Inv. & VQ & DQ & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\multicolumn{13}{l}{\textbf{商业网页}}\\
M1 & 55.4 & 100.0\% & 0.689 & 0.371 & 0.951 & 4.821 & 3.740 & 0.689 & 0.371 & 0.951 & 4.821 & 3.740\\
M2 & 88.9 & 100.0\% & 0.810 & 0.590 & 0.944 & 4.770 & 4.010 & 0.810 & 0.590 & 0.944 & 4.770 & 4.010\\
M3 & 119.6 & 100.0\% & 0.785 & 0.448 & 0.971 & 4.689 & 4.005 & 0.785 & 0.448 & 0.971 & 4.689 & 4.005\\
M4 & 91.9 & 99.0\% & 0.795 & 0.445 & 0.932 & 4.740 & 3.974 & 0.805 & 0.454 & 0.944 & 4.789 & 4.016\\
M5 & 368.8 & 83.7\% & 0.640 & 0.345 & 0.760 & 4.036 & 3.454 & 0.816 & 0.455 & 0.935 & 4.823 & 4.128\\
M6 & 274.6 & 100.0\% & 0.770 & 0.465 & 0.978 & 4.852 & 4.026 & 0.770 & 0.465 & 0.978 & 4.852 & 4.026\\
M7 & 1018.6 & 95.4\% & 0.752 & 0.445 & 0.978 & 4.816 & 4.026 & 0.754 & 0.445 & 0.981 & 4.841 & 4.046\\
M8 & 388.6 & 83.2\% & 0.765 & 0.442 & 0.949 & 4.383 & 3.806 & 0.765 & 0.442 & 0.949 & 4.383 & 3.806\\
M9 & 876.6 & 98.5\% & 0.780 & 0.471 & 0.980 & 4.857 & 4.051 & 0.780 & 0.471 & 0.980 & 4.857 & 4.051\\
M10 & 600.1 & 0.0\% & 0.240 & 0.143 & 0.371 & 2.083 & 1.583 & 0.600 & 0.375 & 0.929 & 5.000 & 3.800\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{科研文档}}\\
M1 & 59.3 & 100.0\% & 0.724 & 0.515 & 0.921 & 4.417 & 3.583 & 0.724 & 0.515 & 0.921 & 4.417 & 3.583\\
M2 & 90.6 & 100.0\% & 0.748 & 0.671 & 0.939 & 4.331 & 3.957 & 0.748 & 0.671 & 0.939 & 4.331 & 3.957\\
M3 & 111.4 & 100.0\% & 0.784 & 0.662 & 0.980 & 4.345 & 4.043 & 0.784 & 0.662 & 0.980 & 4.345 & 4.043\\
M4 & 121.5 & 99.3\% & 0.781 & 0.649 & 0.912 & 4.504 & 3.978 & 0.789 & 0.658 & 0.918 & 4.536 & 4.007\\
M5 & 419.3 & 64.7\% & 0.515 & 0.416 & 0.606 & 2.986 & 2.640 & 0.818 & 0.686 & 0.961 & 4.611 & 4.078\\
M6 & 296.6 & 99.3\% & 0.811 & 0.688 & 0.986 & 4.561 & 4.043 & 0.811 & 0.688 & 0.986 & 4.561 & 4.043\\
M7 & 1448.2 & 61.9\% & 0.744 & 0.563 & 0.941 & 4.338 & 3.827 & 0.786 & 0.602 & 0.984 & 4.534 & 4.000\\
M8 & 452.2 & 61.9\% & 0.748 & 0.584 & 0.898 & 3.849 & 3.611 & 0.776 & 0.603 & 0.934 & 4.023 & 3.774\\
M9 & 1414.8 & 66.2\% & 0.744 & 0.602 & 0.921 & 4.338 & 3.878 & 0.781 & 0.626 & 0.971 & 4.568 & 4.083\\
M10 & 600.1 & 0.0\% & 0.037 & 0.048 & 0.167 & 0.583 & 0.583 & 0.250 & 0.333 & 1.000 & 3.500 & 3.500\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{交互数据面板}}\\
M1 & 53.5 & 100.0\% & 0.702 & 0.381 & 0.956 & 4.651 & 3.413 & 0.702 & 0.381 & 0.956 & 4.651 & 3.413\\
M2 & 86.7 & 100.0\% & 0.808 & 0.570 & 0.958 & 4.607 & 3.817 & 0.808 & 0.570 & 0.958 & 4.607 & 3.817\\
M3 & 112.6 & 100.0\% & 0.740 & 0.492 & 0.986 & 4.539 & 3.869 & 0.740 & 0.492 & 0.986 & 4.539 & 3.869\\
M4 & 114.0 & 100.0\% & 0.743 & 0.495 & 0.929 & 4.723 & 3.885 & 0.743 & 0.495 & 0.929 & 4.723 & 3.885\\
M5 & 362.4 & 77.0\% & 0.621 & 0.455 & 0.718 & 3.618 & 3.204 & 0.837 & 0.608 & 0.941 & 4.701 & 4.163\\
M6 & 300.5 & 97.9\% & 0.735 & 0.517 & 0.991 & 4.639 & 3.979 & 0.735 & 0.517 & 0.991 & 4.639 & 3.979\\
M7 & 992.5 & 95.3\% & 0.738 & 0.505 & 0.977 & 4.670 & 3.895 & 0.745 & 0.506 & 0.989 & 4.720 & 3.937\\
M8 & 442.8 & 65.4\% & 0.798 & 0.595 & 0.929 & 4.225 & 3.927 & 0.804 & 0.595 & 0.937 & 4.270 & 3.968\\
M9 & 968.0 & 94.2\% & 0.745 & 0.505 & 0.986 & 4.702 & 3.916 & 0.745 & 0.505 & 0.986 & 4.702 & 3.916\\
M10 & 600.1 & 0.0\% & 0.148 & 0.174 & 0.457 & 2.000 & 1.500 & 0.308 & 0.364 & 1.000 & 4.800 & 3.600\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{流程与工作流}}\\
M1 & 56.9 & 100.0\% & 0.721 & 0.632 & 0.898 & 4.240 & 3.969 & 0.721 & 0.632 & 0.898 & 4.240 & 3.969\\
M2 & 50.1 & 59.4\% & 0.478 & 0.443 & 0.580 & 2.642 & 2.576 & 0.785 & 0.704 & 0.968 & 4.449 & 4.338\\
M3 & 120.8 & 98.3\% & 0.803 & 0.724 & 0.891 & 3.852 & 3.974 & 0.827 & 0.747 & 0.911 & 3.920 & 4.044\\
M4 & 93.2 & 96.5\% & 0.771 & 0.710 & 0.815 & 3.747 & 3.664 & 0.795 & 0.733 & 0.844 & 3.882 & 3.796\\
M5 & 429.4 & 44.1\% & 0.367 & 0.329 & 0.394 & 1.847 & 1.939 & 0.832 & 0.761 & 0.910 & 4.188 & 4.396\\
M6 & 384.6 & 88.6\% & 0.812 & 0.774 & 0.913 & 4.096 & 4.175 & 0.827 & 0.790 & 0.926 & 4.150 & 4.230\\
M7 & 1366.5 & 60.3\% & 0.555 & 0.557 & 0.679 & 3.140 & 3.070 & 0.741 & 0.719 & 0.937 & 4.331 & 4.235\\
M8 & 469.2 & 48.0\% & 0.666 & 0.632 & 0.748 & 3.262 & 3.432 & 0.774 & 0.739 & 0.873 & 3.831 & 4.031\\
M9 & 1380.2 & 64.6\% & 0.607 & 0.605 & 0.740 & 3.428 & 3.376 & 0.743 & 0.731 & 0.932 & 4.386 & 4.318\\
M10 & 600.1 & 0.0\% & 0.077 & 0.091 & 0.108 & 0.667 & 0.833 & 0.667 & 1.000 & 0.667 & 4.000 & 5.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{系统与架构}}\\
M1 & 52.0 & 100.0\% & 0.798 & 0.628 & 0.820 & 4.246 & 4.246 & 0.798 & 0.628 & 0.820 & 4.246 & 4.246\\
M2 & 79.9 & 100.0\% & 0.813 & 0.660 & 0.960 & 4.373 & 4.470 & 0.813 & 0.660 & 0.960 & 4.373 & 4.470\\
M3 & 96.8 & 88.1\% & 0.786 & 0.654 & 0.719 & 2.448 & 3.761 & 0.882 & 0.724 & 0.820 & 2.780 & 4.271\\
M4 & 170.4 & 85.8\% & 0.739 & 0.612 & 0.716 & 3.239 & 3.657 & 0.892 & 0.757 & 0.842 & 3.774 & 4.261\\
M5 & 536.8 & 23.9\% & 0.179 & 0.165 & 0.201 & 0.881 & 1.060 & 0.821 & 0.756 & 0.852 & 3.688 & 4.438\\
M6 & 269.5 & 98.5\% & 0.872 & 0.734 & 0.903 & 3.806 & 4.508 & 0.875 & 0.734 & 0.908 & 3.835 & 4.541\\
M7 & 1244.8 & 67.2\% & 0.728 & 0.601 & 0.785 & 3.724 & 3.910 & 0.827 & 0.689 & 0.913 & 4.265 & 4.479\\
M8 & 460.3 & 58.2\% & 0.802 & 0.702 & 0.794 & 3.351 & 3.955 & 0.831 & 0.725 & 0.825 & 3.508 & 4.141\\
M9 & 1368.6 & 61.9\% & 0.685 & 0.564 & 0.775 & 3.590 & 3.791 & 0.800 & 0.675 & 0.897 & 4.111 & 4.342\\
M10 & 600.1 & 0.0\% & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\addlinespace[2pt]
\bottomrule\end{tabular}\endgroup

==> tables/compact_results_2.tex <==
\begingroup\fontsize{7.2}{8.4}\selectfont\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{@{}lrr*{10}{r}@{}}\toprule
 & & & \multicolumn{5}{c}{Auto-zero} & \multicolumn{5}{c}{Completed-only}\\
ID & 秒 & 完成率 & Dir. & Der. & Inv. & VQ & DQ & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\multicolumn{13}{l}{\textbf{电路与逻辑}}\\
M1 & 44.4 & 100.0\% & 0.720 & 0.659 & 0.952 & 4.385 & 3.975 & 0.720 & 0.659 & 0.952 & 4.385 & 3.975\\
M2 & 72.5 & 100.0\% & 0.781 & 0.731 & 0.963 & 4.435 & 4.062 & 0.781 & 0.731 & 0.963 & 4.435 & 4.062\\
M3 & 73.7 & 90.7\% & 0.695 & 0.659 & 0.837 & 3.106 & 3.689 & 0.774 & 0.742 & 0.927 & 3.425 & 4.069\\
M4 & 181.9 & 84.5\% & 0.649 & 0.560 & 0.743 & 3.410 & 3.280 & 0.786 & 0.698 & 0.894 & 4.037 & 3.882\\
M5 & 548.3 & 18.0\% & 0.141 & 0.121 & 0.160 & 0.814 & 0.758 & 0.815 & 0.730 & 0.961 & 4.517 & 4.207\\
M6 & 200.8 & 95.0\% & 0.781 & 0.771 & 0.925 & 4.118 & 4.143 & 0.805 & 0.785 & 0.959 & 4.305 & 4.331\\
M7 & 950.2 & 87.6\% & 0.727 & 0.686 & 0.905 & 4.168 & 4.106 & 0.774 & 0.725 & 0.958 & 4.415 & 4.349\\
M8 & 430.3 & 66.5\% & 0.704 & 0.682 & 0.873 & 3.404 & 3.584 & 0.718 & 0.697 & 0.894 & 3.490 & 3.675\\
M9 & 1083.3 & 80.1\% & 0.720 & 0.668 & 0.877 & 3.907 & 3.708 & 0.786 & 0.720 & 0.961 & 4.308 & 4.089\\
M10 & 600.1 & 0.0\% & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{科研统计图}}\\
M1 & 55.6 & 100.0\% & 0.815 & 0.502 & 0.949 & 4.258 & 3.450 & 0.815 & 0.502 & 0.949 & 4.258 & 3.450\\
M2 & 83.6 & 100.0\% & 0.861 & 0.648 & 0.966 & 4.291 & 3.907 & 0.861 & 0.648 & 0.966 & 4.291 & 3.907\\
M3 & 94.1 & 99.3\% & 0.904 & 0.736 & 0.981 & 4.046 & 4.311 & 0.913 & 0.749 & 0.987 & 4.073 & 4.340\\
M4 & 89.2 & 99.3\% & 0.911 & 0.728 & 0.928 & 3.861 & 4.066 & 0.914 & 0.728 & 0.934 & 3.887 & 4.093\\
M5 & 478.4 & 50.3\% & 0.457 & 0.347 & 0.487 & 2.086 & 2.093 & 0.945 & 0.709 & 0.962 & 4.145 & 4.158\\
M6 & 286.8 & 99.3\% & 0.924 & 0.736 & 0.992 & 4.404 & 4.364 & 0.924 & 0.736 & 0.992 & 4.404 & 4.364\\
M7 & 917.1 & 94.0\% & 0.914 & 0.766 & 0.970 & 4.517 & 4.338 & 0.914 & 0.766 & 0.970 & 4.517 & 4.338\\
M8 & 447.0 & 62.3\% & 0.834 & 0.682 & 0.877 & 3.444 & 3.762 & 0.875 & 0.712 & 0.920 & 3.586 & 3.917\\
M9 & 990.1 & 85.4\% & 0.904 & 0.745 & 0.992 & 4.589 & 4.344 & 0.904 & 0.745 & 0.992 & 4.589 & 4.344\\
M10 & 600.1 & 0.0\% & 0.200 & 0.200 & 0.231 & 1.083 & 1.083 & 1.000 & 1.000 & 1.000 & 4.333 & 4.333\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{数学与几何}}\\
M1 & 46.3 & 100.0\% & 0.664 & 0.390 & 0.877 & 4.263 & 3.359 & 0.664 & 0.390 & 0.877 & 4.263 & 3.359\\
M2 & 72.8 & 100.0\% & 0.794 & 0.641 & 0.912 & 4.174 & 3.701 & 0.794 & 0.641 & 0.912 & 4.174 & 3.701\\
M3 & 92.4 & 95.8\% & 0.918 & 0.896 & 0.942 & 4.245 & 4.677 & 0.965 & 0.932 & 0.981 & 4.431 & 4.881\\
M4 & 114.5 & 95.2\% & 0.876 & 0.876 & 0.817 & 3.826 & 4.198 & 0.923 & 0.923 & 0.861 & 4.019 & 4.409\\
M5 & 457.7 & 46.1\% & 0.394 & 0.351 & 0.410 & 1.964 & 2.084 & 0.935 & 0.892 & 0.915 & 4.260 & 4.519\\
M6 & 219.5 & 99.4\% & 0.949 & 0.919 & 0.976 & 4.539 & 4.796 & 0.954 & 0.922 & 0.982 & 4.566 & 4.825\\
M7 & 1059.6 & 89.2\% & 0.924 & 0.896 & 0.970 & 4.545 & 4.761 & 0.941 & 0.917 & 0.990 & 4.628 & 4.848\\
M8 & 394.7 & 78.4\% & 0.885 & 0.788 & 0.877 & 3.826 & 4.000 & 0.901 & 0.797 & 0.895 & 3.896 & 4.073\\
M9 & 1164.7 & 74.9\% & 0.903 & 0.861 & 0.974 & 4.491 & 4.677 & 0.920 & 0.875 & 0.988 & 4.545 & 4.733\\
M10 & 600.1 & 0.0\% & 0.043 & 0.000 & 0.077 & 0.417 & 0.417 & 1.000 & 0.000 & 1.000 & 5.000 & 5.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{化学分子图}}\\
M1 & 40.1 & 100.0\% & 0.770 & 0.706 & 0.903 & 4.785 & 4.278 & 0.770 & 0.706 & 0.903 & 4.785 & 4.278\\
M2 & 66.4 & 99.0\% & 0.809 & 0.752 & 0.927 & 4.566 & 4.258 & 0.826 & 0.773 & 0.939 & 4.611 & 4.301\\
M3 & 72.1 & 99.5\% & 0.850 & 0.752 & 0.954 & 4.688 & 4.488 & 0.854 & 0.752 & 0.958 & 4.711 & 4.510\\
M4 & 114.5 & 90.2\% & 0.745 & 0.636 & 0.650 & 3.668 & 3.615 & 0.839 & 0.711 & 0.722 & 4.065 & 4.005\\
M5 & 496.7 & 37.6\% & 0.306 & 0.280 & 0.292 & 1.532 & 1.566 & 0.845 & 0.748 & 0.784 & 4.078 & 4.169\\
M6 & 176.1 & 97.6\% & 0.821 & 0.755 & 0.951 & 4.707 & 4.561 & 0.839 & 0.769 & 0.975 & 4.825 & 4.675\\
M7 & 801.0 & 89.8\% & 0.827 & 0.734 & 0.941 & 4.644 & 4.517 & 0.839 & 0.739 & 0.964 & 4.760 & 4.630\\
M8 & 438.8 & 67.3\% & 0.765 & 0.668 & 0.784 & 3.971 & 3.795 & 0.833 & 0.707 & 0.855 & 4.376 & 4.183\\
M9 & 793.9 & 90.7\% & 0.842 & 0.745 & 0.966 & 4.737 & 4.473 & 0.851 & 0.753 & 0.981 & 4.807 & 4.540\\
M10 & 540.4 & 41.7\% & 0.318 & 0.143 & 0.457 & 2.417 & 2.167 & 0.875 & 0.500 & 1.000 & 4.833 & 4.333\\
\addlinespace[2pt]
\bottomrule\end{tabular}\endgroup

==> tables/compact_results_3.tex <==
\begingroup\fontsize{6.2}{6.9}\selectfont\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{0.72}
\begin{tabular}{@{}lrr*{10}{r}@{}}\toprule
 & & & \multicolumn{5}{c}{Auto-zero} & \multicolumn{5}{c}{Completed-only}\\
ID & 秒 & 完成率 & Dir. & Der. & Inv. & VQ & DQ & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\multicolumn{13}{l}{\textbf{Easy}}\\
M1 & 50.1 & 100.0\% & 0.897 & 0.556 & 0.929 & 4.570 & 4.520 & 0.897 & 0.556 & 0.929 & 4.570 & 4.520\\
M2 & 70.0 & 93.3\% & 0.884 & 0.667 & 0.900 & 4.300 & 4.338 & 0.939 & 0.667 & 0.967 & 4.607 & 4.648\\
M3 & 102.4 & 97.0\% & 0.916 & 0.556 & 0.920 & 4.115 & 4.368 & 0.943 & 0.556 & 0.946 & 4.242 & 4.503\\
M4 & 113.1 & 95.3\% & 0.909 & 0.556 & 0.810 & 4.027 & 4.097 & 0.954 & 0.625 & 0.852 & 4.224 & 4.297\\
M5 & 434.9 & 52.0\% & 0.501 & 0.556 & 0.457 & 2.327 & 2.363 & 0.958 & 1.000 & 0.889 & 4.474 & 4.545\\
M6 & 282.7 & 95.3\% & 0.933 & 0.667 & 0.946 & 4.480 & 4.592 & 0.944 & 0.667 & 0.957 & 4.540 & 4.654\\
M7 & 1125.4 & 79.2\% & 0.850 & 0.667 & 0.878 & 4.293 & 4.308 & 0.917 & 0.667 & 0.962 & 4.684 & 4.700\\
M8 & 463.4 & 56.8\% & 0.863 & 0.667 & 0.811 & 3.752 & 3.997 & 0.920 & 0.667 & 0.867 & 4.005 & 4.267\\
M9 & 1161.3 & 76.5\% & 0.877 & 0.667 & 0.900 & 4.345 & 4.372 & 0.931 & 0.667 & 0.963 & 4.639 & 4.667\\
M10 & 586.9 & 5.6\% & 0.209 & 0.000 & 0.286 & 1.361 & 1.222 & 0.818 & 0.000 & 1.000 & 4.900 & 4.400\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Medium}}\\
M1 & 51.1 & 100.0\% & 0.772 & 0.546 & 0.925 & 4.413 & 3.616 & 0.772 & 0.546 & 0.925 & 4.413 & 3.616\\
M2 & 74.9 & 94.7\% & 0.777 & 0.640 & 0.898 & 4.176 & 3.764 & 0.820 & 0.677 & 0.950 & 4.408 & 3.972\\
M3 & 98.9 & 97.7\% & 0.846 & 0.656 & 0.933 & 4.036 & 4.002 & 0.866 & 0.670 & 0.954 & 4.129 & 4.094\\
M4 & 119.6 & 94.9\% & 0.826 & 0.619 & 0.833 & 3.993 & 3.707 & 0.870 & 0.651 & 0.878 & 4.205 & 3.905\\
M5 & 449.4 & 52.2\% & 0.457 & 0.336 & 0.487 & 2.330 & 2.161 & 0.875 & 0.637 & 0.928 & 4.468 & 4.144\\
M6 & 267.0 & 97.7\% & 0.863 & 0.680 & 0.959 & 4.402 & 4.086 & 0.875 & 0.688 & 0.971 & 4.460 & 4.141\\
M7 & 1069.6 & 84.2\% & 0.818 & 0.605 & 0.916 & 4.285 & 3.989 & 0.867 & 0.641 & 0.974 & 4.541 & 4.227\\
M8 & 437.0 & 67.5\% & 0.789 & 0.603 & 0.870 & 3.728 & 3.623 & 0.832 & 0.637 & 0.914 & 3.927 & 3.816\\
M9 & 1099.7 & 82.0\% & 0.804 & 0.600 & 0.905 & 4.255 & 3.865 & 0.859 & 0.641 & 0.971 & 4.563 & 4.145\\
M10 & 593.4 & 8.3\% & 0.174 & 0.200 & 0.224 & 1.028 & 1.056 & 0.706 & 0.733 & 0.889 & 4.111 & 4.222\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Hard}}\\
M1 & 53.4 & 100.0\% & 0.622 & 0.515 & 0.895 & 4.396 & 3.000 & 0.622 & 0.515 & 0.895 & 4.396 & 3.000\\
M2 & 83.9 & 93.9\% & 0.682 & 0.611 & 0.872 & 4.084 & 3.136 & 0.729 & 0.651 & 0.931 & 4.351 & 3.341\\
M3 & 98.2 & 96.8\% & 0.728 & 0.668 & 0.921 & 4.002 & 3.845 & 0.754 & 0.691 & 0.952 & 4.134 & 3.972\\
M4 & 124.0 & 93.4\% & 0.683 & 0.639 & 0.835 & 3.927 & 3.530 & 0.733 & 0.683 & 0.891 & 4.204 & 3.779\\
M5 & 473.5 & 46.1\% & 0.345 & 0.313 & 0.429 & 2.018 & 1.770 & 0.767 & 0.678 & 0.941 & 4.374 & 3.837\\
M6 & 257.1 & 98.2\% & 0.747 & 0.709 & 0.966 & 4.400 & 4.091 & 0.751 & 0.712 & 0.971 & 4.420 & 4.110\\
M7 & 1039.8 & 85.2\% & 0.676 & 0.643 & 0.907 & 4.229 & 3.677 & 0.721 & 0.684 & 0.966 & 4.495 & 3.908\\
M8 & 396.3 & 75.2\% & 0.713 & 0.652 & 0.883 & 3.818 & 3.582 & 0.738 & 0.675 & 0.915 & 3.953 & 3.708\\
M9 & 1025.1 & 83.9\% & 0.687 & 0.655 & 0.928 & 4.289 & 3.704 & 0.720 & 0.685 & 0.971 & 4.493 & 3.881\\
M10 & 600.1 & 0.0\% & 0.042 & 0.040 & 0.129 & 0.694 & 0.444 & 0.312 & 0.312 & 1.000 & 5.000 & 3.200\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{HTML}}\\
M1 & 55.8 & 100.0\% & 0.703 & 0.414 & 0.944 & 4.653 & 3.580 & 0.703 & 0.414 & 0.944 & 4.653 & 3.580\\
M2 & 88.6 & 100.0\% & 0.793 & 0.604 & 0.948 & 4.595 & 3.926 & 0.793 & 0.604 & 0.948 & 4.595 & 3.926\\
M3 & 114.9 & 100.0\% & 0.768 & 0.522 & 0.979 & 4.544 & 3.966 & 0.768 & 0.522 & 0.979 & 4.544 & 3.966\\
M4 & 107.7 & 99.4\% & 0.772 & 0.519 & 0.925 & 4.671 & 3.943 & 0.777 & 0.524 & 0.931 & 4.698 & 3.966\\
M5 & 379.8 & 76.2\% & 0.600 & 0.405 & 0.703 & 3.607 & 3.148 & 0.824 & 0.568 & 0.943 & 4.731 & 4.130\\
M6 & 289.8 & 99.0\% & 0.768 & 0.544 & 0.985 & 4.698 & 4.013 & 0.768 & 0.544 & 0.985 & 4.698 & 4.013\\
M7 & 1122.7 & 86.5\% & 0.745 & 0.499 & 0.968 & 4.637 & 3.926 & 0.759 & 0.508 & 0.985 & 4.718 & 3.994\\
M8 & 425.1 & 71.1\% & 0.773 & 0.537 & 0.928 & 4.184 & 3.799 & 0.783 & 0.541 & 0.941 & 4.249 & 3.857\\
M9 & 1052.0 & 88.4\% & 0.757 & 0.519 & 0.966 & 4.663 & 3.956 & 0.767 & 0.524 & 0.980 & 4.726 & 4.010\\
M10 & 600.1 & 0.0\% & 0.139 & 0.123 & 0.330 & 1.556 & 1.222 & 0.407 & 0.364 & 0.972 & 4.667 & 3.667\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{DOT}}\\
M1 & 56.9 & 100.0\% & 0.721 & 0.632 & 0.898 & 4.240 & 3.969 & 0.721 & 0.632 & 0.898 & 4.240 & 3.969\\
M2 & 50.1 & 59.4\% & 0.478 & 0.443 & 0.580 & 2.642 & 2.576 & 0.785 & 0.704 & 0.968 & 4.449 & 4.338\\
M3 & 120.8 & 98.3\% & 0.803 & 0.724 & 0.891 & 3.852 & 3.974 & 0.827 & 0.747 & 0.911 & 3.920 & 4.044\\
M4 & 93.2 & 96.5\% & 0.771 & 0.710 & 0.815 & 3.747 & 3.664 & 0.795 & 0.733 & 0.844 & 3.882 & 3.796\\
M5 & 429.4 & 44.1\% & 0.367 & 0.329 & 0.394 & 1.847 & 1.939 & 0.832 & 0.761 & 0.910 & 4.188 & 4.396\\
M6 & 384.6 & 88.6\% & 0.812 & 0.774 & 0.913 & 4.096 & 4.175 & 0.827 & 0.790 & 0.926 & 4.150 & 4.230\\
M7 & 1366.5 & 60.3\% & 0.555 & 0.557 & 0.679 & 3.140 & 3.070 & 0.741 & 0.719 & 0.937 & 4.331 & 4.235\\
M8 & 469.2 & 48.0\% & 0.666 & 0.632 & 0.748 & 3.262 & 3.432 & 0.774 & 0.739 & 0.873 & 3.831 & 4.031\\
M9 & 1380.2 & 64.6\% & 0.607 & 0.605 & 0.740 & 3.428 & 3.376 & 0.743 & 0.731 & 0.932 & 4.386 & 4.318\\
M10 & 600.1 & 0.0\% & 0.077 & 0.091 & 0.108 & 0.667 & 0.833 & 0.667 & 1.000 & 0.667 & 4.000 & 5.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{TikZ}}\\
M1 & 52.0 & 100.0\% & 0.798 & 0.628 & 0.820 & 4.246 & 4.246 & 0.798 & 0.628 & 0.820 & 4.246 & 4.246\\
M2 & 79.9 & 100.0\% & 0.813 & 0.660 & 0.960 & 4.373 & 4.470 & 0.813 & 0.660 & 0.960 & 4.373 & 4.470\\
M3 & 96.8 & 88.1\% & 0.786 & 0.654 & 0.719 & 2.448 & 3.761 & 0.882 & 0.724 & 0.820 & 2.780 & 4.271\\
M4 & 170.4 & 85.8\% & 0.739 & 0.612 & 0.716 & 3.239 & 3.657 & 0.892 & 0.757 & 0.842 & 3.774 & 4.261\\
M5 & 536.8 & 23.9\% & 0.179 & 0.165 & 0.201 & 0.881 & 1.060 & 0.821 & 0.756 & 0.852 & 3.688 & 4.438\\
M6 & 269.5 & 98.5\% & 0.872 & 0.734 & 0.903 & 3.806 & 4.508 & 0.875 & 0.734 & 0.908 & 3.835 & 4.541\\
M7 & 1244.8 & 67.2\% & 0.728 & 0.601 & 0.785 & 3.724 & 3.910 & 0.827 & 0.689 & 0.913 & 4.265 & 4.479\\
M8 & 460.3 & 58.2\% & 0.802 & 0.702 & 0.794 & 3.351 & 3.955 & 0.831 & 0.725 & 0.825 & 3.508 & 4.141\\
M9 & 1368.6 & 61.9\% & 0.685 & 0.564 & 0.775 & 3.590 & 3.791 & 0.800 & 0.675 & 0.897 & 4.111 & 4.342\\
M10 & 600.1 & 0.0\% & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{CircuitikZ}}\\
M1 & 44.4 & 100.0\% & 0.720 & 0.659 & 0.952 & 4.385 & 3.975 & 0.720 & 0.659 & 0.952 & 4.385 & 3.975\\
M2 & 72.5 & 100.0\% & 0.781 & 0.731 & 0.963 & 4.435 & 4.062 & 0.781 & 0.731 & 0.963 & 4.435 & 4.062\\
M3 & 73.7 & 90.7\% & 0.695 & 0.659 & 0.837 & 3.106 & 3.689 & 0.774 & 0.742 & 0.927 & 3.425 & 4.069\\
M4 & 181.9 & 84.5\% & 0.649 & 0.560 & 0.743 & 3.410 & 3.280 & 0.786 & 0.698 & 0.894 & 4.037 & 3.882\\
M5 & 548.3 & 18.0\% & 0.141 & 0.121 & 0.160 & 0.814 & 0.758 & 0.815 & 0.730 & 0.961 & 4.517 & 4.207\\
M6 & 200.8 & 95.0\% & 0.781 & 0.771 & 0.925 & 4.118 & 4.143 & 0.805 & 0.785 & 0.959 & 4.305 & 4.331\\
M7 & 950.2 & 87.6\% & 0.727 & 0.686 & 0.905 & 4.168 & 4.106 & 0.774 & 0.725 & 0.958 & 4.415 & 4.349\\
M8 & 430.3 & 66.5\% & 0.704 & 0.682 & 0.873 & 3.404 & 3.584 & 0.718 & 0.697 & 0.894 & 3.490 & 3.675\\
M9 & 1083.3 & 80.1\% & 0.720 & 0.668 & 0.877 & 3.907 & 3.708 & 0.786 & 0.720 & 0.961 & 4.308 & 4.089\\
M10 & 600.1 & 0.0\% & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Python}}\\
M1 & 46.6 & 100.0\% & 0.749 & 0.539 & 0.908 & 4.466 & 3.746 & 0.749 & 0.539 & 0.908 & 4.466 & 3.746\\
M2 & 73.4 & 99.6\% & 0.819 & 0.684 & 0.934 & 4.361 & 3.979 & 0.826 & 0.691 & 0.938 & 4.378 & 3.994\\
M3 & 84.9 & 98.3\% & 0.888 & 0.795 & 0.958 & 4.361 & 4.497 & 0.906 & 0.809 & 0.974 & 4.438 & 4.576\\
M4 & 107.2 & 94.5\% & 0.836 & 0.744 & 0.782 & 3.774 & 3.931 & 0.890 & 0.787 & 0.830 & 3.996 & 4.162\\
M5 & 479.0 & 44.0\% & 0.379 & 0.324 & 0.385 & 1.830 & 1.883 & 0.909 & 0.779 & 0.886 & 4.161 & 4.283\\
M6 & 221.9 & 98.7\% & 0.893 & 0.804 & 0.970 & 4.566 & 4.579 & 0.901 & 0.810 & 0.982 & 4.619 & 4.633\\
M7 & 917.1 & 90.8\% & 0.884 & 0.797 & 0.959 & 4.575 & 4.543 & 0.894 & 0.805 & 0.974 & 4.647 & 4.614\\
M8 & 427.1 & 69.4\% & 0.824 & 0.712 & 0.840 & 3.772 & 3.851 & 0.868 & 0.739 & 0.887 & 3.986 & 4.069\\
M9 & 968.9 & 84.1\% & 0.880 & 0.783 & 0.976 & 4.616 & 4.501 & 0.889 & 0.790 & 0.986 & 4.660 & 4.544\\
M10 & 580.2 & 13.9\% & 0.186 & 0.109 & 0.248 & 1.306 & 1.222 & 0.929 & 0.750 & 1.000 & 4.700 & 4.400\\
\addlinespace[2pt]
\bottomrule\end{tabular}\endgroup

==> tables/compact_results_3_en.tex <==
\begingroup\fontsize{7.2}{8.4}\selectfont\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{0.90}
\begin{tabular}{@{}lrr*{10}{r}@{}}\toprule
 & & & \multicolumn{5}{c}{Auto-zero} & \multicolumn{5}{c}{Completed-only}\\
ID & Time (s) & Completion & Dir. & Der. & Inv. & VQ & DQ & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\multicolumn{13}{l}{\textbf{Easy}}\\
M1 & 50.1 & 100.0\% & 0.897 & 0.556 & 0.929 & 4.570 & 4.520 & 0.897 & 0.556 & 0.929 & 4.570 & 4.520\\
M2 & 70.0 & 93.3\% & 0.884 & 0.667 & 0.900 & 4.300 & 4.338 & 0.939 & 0.667 & 0.967 & 4.607 & 4.648\\
M3 & 102.4 & 97.0\% & 0.916 & 0.556 & 0.920 & 4.115 & 4.368 & 0.943 & 0.556 & 0.946 & 4.242 & 4.503\\
M4 & 113.1 & 95.3\% & 0.909 & 0.556 & 0.810 & 4.027 & 4.097 & 0.954 & 0.625 & 0.852 & 4.224 & 4.297\\
M5 & 434.9 & 52.0\% & 0.501 & 0.556 & 0.457 & 2.327 & 2.363 & 0.958 & 1.000 & 0.889 & 4.474 & 4.545\\
M6 & 282.7 & 95.3\% & 0.933 & 0.667 & 0.946 & 4.480 & 4.592 & 0.944 & 0.667 & 0.957 & 4.540 & 4.654\\
M7 & 463.4 & 56.8\% & 0.863 & 0.667 & 0.811 & 3.752 & 3.997 & 0.920 & 0.667 & 0.867 & 4.005 & 4.267\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Medium}}\\
M1 & 51.1 & 100.0\% & 0.772 & 0.546 & 0.925 & 4.413 & 3.616 & 0.772 & 0.546 & 0.925 & 4.413 & 3.616\\
M2 & 74.9 & 94.7\% & 0.777 & 0.640 & 0.898 & 4.176 & 3.764 & 0.820 & 0.677 & 0.950 & 4.408 & 3.972\\
M3 & 98.9 & 97.7\% & 0.846 & 0.656 & 0.933 & 4.036 & 4.002 & 0.866 & 0.670 & 0.954 & 4.129 & 4.094\\
M4 & 119.6 & 94.9\% & 0.826 & 0.619 & 0.833 & 3.993 & 3.707 & 0.870 & 0.651 & 0.878 & 4.205 & 3.905\\
M5 & 449.4 & 52.2\% & 0.457 & 0.336 & 0.487 & 2.330 & 2.161 & 0.875 & 0.637 & 0.928 & 4.468 & 4.144\\
M6 & 267.0 & 97.7\% & 0.863 & 0.680 & 0.959 & 4.402 & 4.086 & 0.875 & 0.688 & 0.971 & 4.460 & 4.141\\
M7 & 437.0 & 67.5\% & 0.789 & 0.603 & 0.870 & 3.728 & 3.623 & 0.832 & 0.637 & 0.914 & 3.927 & 3.816\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Hard}}\\
M1 & 53.4 & 100.0\% & 0.622 & 0.515 & 0.895 & 4.396 & 3.000 & 0.622 & 0.515 & 0.895 & 4.396 & 3.000\\
M2 & 83.9 & 93.9\% & 0.682 & 0.611 & 0.872 & 4.084 & 3.136 & 0.729 & 0.651 & 0.931 & 4.351 & 3.341\\
M3 & 98.2 & 96.8\% & 0.728 & 0.668 & 0.921 & 4.002 & 3.845 & 0.754 & 0.691 & 0.952 & 4.134 & 3.972\\
M4 & 124.0 & 93.4\% & 0.683 & 0.639 & 0.835 & 3.927 & 3.530 & 0.733 & 0.683 & 0.891 & 4.204 & 3.779\\
M5 & 473.5 & 46.1\% & 0.345 & 0.313 & 0.429 & 2.018 & 1.770 & 0.767 & 0.678 & 0.941 & 4.374 & 3.837\\
M6 & 257.1 & 98.2\% & 0.747 & 0.709 & 0.966 & 4.400 & 4.091 & 0.751 & 0.712 & 0.971 & 4.420 & 4.110\\
M7 & 396.3 & 75.2\% & 0.713 & 0.652 & 0.883 & 3.818 & 3.582 & 0.738 & 0.675 & 0.915 & 3.953 & 3.708\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{HTML}}\\
M1 & 55.8 & 100.0\% & 0.703 & 0.414 & 0.944 & 4.653 & 3.580 & 0.703 & 0.414 & 0.944 & 4.653 & 3.580\\
M2 & 88.6 & 100.0\% & 0.793 & 0.604 & 0.948 & 4.595 & 3.926 & 0.793 & 0.604 & 0.948 & 4.595 & 3.926\\
M3 & 114.9 & 100.0\% & 0.768 & 0.522 & 0.979 & 4.544 & 3.966 & 0.768 & 0.522 & 0.979 & 4.544 & 3.966\\
M4 & 107.7 & 99.4\% & 0.772 & 0.519 & 0.925 & 4.671 & 3.943 & 0.777 & 0.524 & 0.931 & 4.698 & 3.966\\
M5 & 379.8 & 76.2\% & 0.600 & 0.405 & 0.703 & 3.607 & 3.148 & 0.824 & 0.568 & 0.943 & 4.731 & 4.130\\
M6 & 289.8 & 99.0\% & 0.768 & 0.544 & 0.985 & 4.698 & 4.013 & 0.768 & 0.544 & 0.985 & 4.698 & 4.013\\
M7 & 425.1 & 71.1\% & 0.773 & 0.537 & 0.928 & 4.184 & 3.799 & 0.783 & 0.541 & 0.941 & 4.249 & 3.857\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{DOT}}\\
M1 & 56.9 & 100.0\% & 0.721 & 0.632 & 0.898 & 4.240 & 3.969 & 0.721 & 0.632 & 0.898 & 4.240 & 3.969\\
M2 & 50.1 & 59.4\% & 0.478 & 0.443 & 0.580 & 2.642 & 2.576 & 0.785 & 0.704 & 0.968 & 4.449 & 4.338\\
M3 & 120.8 & 98.3\% & 0.803 & 0.724 & 0.891 & 3.852 & 3.974 & 0.827 & 0.747 & 0.911 & 3.920 & 4.044\\
M4 & 93.2 & 96.5\% & 0.771 & 0.710 & 0.815 & 3.747 & 3.664 & 0.795 & 0.733 & 0.844 & 3.882 & 3.796\\
M5 & 429.4 & 44.1\% & 0.367 & 0.329 & 0.394 & 1.847 & 1.939 & 0.832 & 0.761 & 0.910 & 4.188 & 4.396\\
M6 & 384.6 & 88.6\% & 0.812 & 0.774 & 0.913 & 4.096 & 4.175 & 0.827 & 0.790 & 0.926 & 4.150 & 4.230\\
M7 & 469.2 & 48.0\% & 0.666 & 0.632 & 0.748 & 3.262 & 3.432 & 0.774 & 0.739 & 0.873 & 3.831 & 4.031\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{TikZ}}\\
M1 & 52.0 & 100.0\% & 0.798 & 0.628 & 0.820 & 4.246 & 4.246 & 0.798 & 0.628 & 0.820 & 4.246 & 4.246\\
M2 & 79.9 & 100.0\% & 0.813 & 0.660 & 0.960 & 4.373 & 4.470 & 0.813 & 0.660 & 0.960 & 4.373 & 4.470\\
M3 & 96.8 & 88.1\% & 0.786 & 0.654 & 0.719 & 2.448 & 3.761 & 0.882 & 0.724 & 0.820 & 2.780 & 4.271\\
M4 & 170.4 & 85.8\% & 0.739 & 0.612 & 0.716 & 3.239 & 3.657 & 0.892 & 0.757 & 0.842 & 3.774 & 4.261\\
M5 & 536.8 & 23.9\% & 0.179 & 0.165 & 0.201 & 0.881 & 1.060 & 0.821 & 0.756 & 0.852 & 3.688 & 4.438\\
M6 & 269.5 & 98.5\% & 0.872 & 0.734 & 0.903 & 3.806 & 4.508 & 0.875 & 0.734 & 0.908 & 3.835 & 4.541\\
M7 & 460.3 & 58.2\% & 0.802 & 0.702 & 0.794 & 3.351 & 3.955 & 0.831 & 0.725 & 0.825 & 3.508 & 4.141\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{CircuitikZ}}\\
M1 & 44.4 & 100.0\% & 0.720 & 0.659 & 0.952 & 4.385 & 3.975 & 0.720 & 0.659 & 0.952 & 4.385 & 3.975\\
M2 & 72.5 & 100.0\% & 0.781 & 0.731 & 0.963 & 4.435 & 4.062 & 0.781 & 0.731 & 0.963 & 4.435 & 4.062\\
M3 & 73.7 & 90.7\% & 0.695 & 0.659 & 0.837 & 3.106 & 3.689 & 0.774 & 0.742 & 0.927 & 3.425 & 4.069\\
M4 & 181.9 & 84.5\% & 0.649 & 0.560 & 0.743 & 3.410 & 3.280 & 0.786 & 0.698 & 0.894 & 4.037 & 3.882\\
M5 & 548.3 & 18.0\% & 0.141 & 0.121 & 0.160 & 0.814 & 0.758 & 0.815 & 0.730 & 0.961 & 4.517 & 4.207\\
M6 & 200.8 & 95.0\% & 0.781 & 0.771 & 0.925 & 4.118 & 4.143 & 0.805 & 0.785 & 0.959 & 4.305 & 4.331\\
M7 & 430.3 & 66.5\% & 0.704 & 0.682 & 0.873 & 3.404 & 3.584 & 0.718 & 0.697 & 0.894 & 3.490 & 3.675\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Python}}\\
M1 & 46.6 & 100.0\% & 0.749 & 0.539 & 0.908 & 4.466 & 3.746 & 0.749 & 0.539 & 0.908 & 4.466 & 3.746\\
M2 & 73.4 & 99.6\% & 0.819 & 0.684 & 0.934 & 4.361 & 3.979 & 0.826 & 0.691 & 0.938 & 4.378 & 3.994\\
M3 & 84.9 & 98.3\% & 0.888 & 0.795 & 0.958 & 4.361 & 4.497 & 0.906 & 0.809 & 0.974 & 4.438 & 4.576\\
M4 & 107.2 & 94.5\% & 0.836 & 0.744 & 0.782 & 3.774 & 3.931 & 0.890 & 0.787 & 0.830 & 3.996 & 4.162\\
M5 & 479.0 & 44.0\% & 0.379 & 0.324 & 0.385 & 1.830 & 1.883 & 0.909 & 0.779 & 0.886 & 4.161 & 4.283\\
M6 & 221.9 & 98.7\% & 0.893 & 0.804 & 0.970 & 4.566 & 4.579 & 0.901 & 0.810 & 0.982 & 4.619 & 4.633\\
M7 & 427.1 & 69.4\% & 0.824 & 0.712 & 0.840 & 3.772 & 3.851 & 0.868 & 0.739 & 0.887 & 3.986 & 4.069\\
\addlinespace[2pt]
\bottomrule\end{tabular}\endgroup


==> tables/compact_results_difficulty.tex <==
\begingroup\fontsize{7.2}{8.4}\selectfont\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{@{}lrr*{10}{r}@{}}\toprule
 & & & \multicolumn{5}{c}{Auto-zero} & \multicolumn{5}{c}{Completed-only}\\
ID & 秒 & 完成率 & Dir. & Der. & Inv. & VQ & DQ & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\multicolumn{13}{l}{\textbf{Easy}}\\
M1 & 50.1 & 100.0\% & 0.897 & 0.556 & 0.929 & 4.570 & 4.520 & 0.897 & 0.556 & 0.929 & 4.570 & 4.520\\
M2 & 70.0 & 93.3\% & 0.884 & 0.667 & 0.900 & 4.300 & 4.338 & 0.939 & 0.667 & 0.967 & 4.607 & 4.648\\
M3 & 102.4 & 97.0\% & 0.916 & 0.556 & 0.920 & 4.115 & 4.368 & 0.943 & 0.556 & 0.946 & 4.242 & 4.503\\
M4 & 113.1 & 95.3\% & 0.909 & 0.556 & 0.810 & 4.027 & 4.097 & 0.954 & 0.625 & 0.852 & 4.224 & 4.297\\
M5 & 434.9 & 52.0\% & 0.501 & 0.556 & 0.457 & 2.327 & 2.363 & 0.958 & 1.000 & 0.889 & 4.474 & 4.545\\
M6 & 282.7 & 95.3\% & 0.933 & 0.667 & 0.946 & 4.480 & 4.592 & 0.944 & 0.667 & 0.957 & 4.540 & 4.654\\
M7 & 1125.4 & 79.2\% & 0.850 & 0.667 & 0.878 & 4.293 & 4.308 & 0.917 & 0.667 & 0.962 & 4.684 & 4.700\\
M8 & 463.4 & 56.8\% & 0.863 & 0.667 & 0.811 & 3.752 & 3.997 & 0.920 & 0.667 & 0.867 & 4.005 & 4.267\\
M9 & 1161.3 & 76.5\% & 0.877 & 0.667 & 0.900 & 4.345 & 4.372 & 0.931 & 0.667 & 0.963 & 4.639 & 4.667\\
M10 & 586.9 & 5.6\% & 0.209 & 0.000 & 0.286 & 1.361 & 1.222 & 0.818 & 0.000 & 1.000 & 4.900 & 4.400\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Medium}}\\
M1 & 51.1 & 100.0\% & 0.772 & 0.546 & 0.925 & 4.413 & 3.616 & 0.772 & 0.546 & 0.925 & 4.413 & 3.616\\
M2 & 74.9 & 94.7\% & 0.777 & 0.640 & 0.898 & 4.176 & 3.764 & 0.820 & 0.677 & 0.950 & 4.408 & 3.972\\
M3 & 98.9 & 97.7\% & 0.846 & 0.656 & 0.933 & 4.036 & 4.002 & 0.866 & 0.670 & 0.954 & 4.129 & 4.094\\
M4 & 119.6 & 94.9\% & 0.826 & 0.619 & 0.833 & 3.993 & 3.707 & 0.870 & 0.651 & 0.878 & 4.205 & 3.905\\
M5 & 449.4 & 52.2\% & 0.457 & 0.336 & 0.487 & 2.330 & 2.161 & 0.875 & 0.637 & 0.928 & 4.468 & 4.144\\
M6 & 267.0 & 97.7\% & 0.863 & 0.680 & 0.959 & 4.402 & 4.086 & 0.875 & 0.688 & 0.971 & 4.460 & 4.141\\
M7 & 1069.6 & 84.2\% & 0.818 & 0.605 & 0.916 & 4.285 & 3.989 & 0.867 & 0.641 & 0.974 & 4.541 & 4.227\\
M8 & 437.0 & 67.5\% & 0.789 & 0.603 & 0.870 & 3.728 & 3.623 & 0.832 & 0.637 & 0.914 & 3.927 & 3.816\\
M9 & 1099.7 & 82.0\% & 0.804 & 0.600 & 0.905 & 4.255 & 3.865 & 0.859 & 0.641 & 0.971 & 4.563 & 4.145\\
M10 & 593.4 & 8.3\% & 0.174 & 0.200 & 0.224 & 1.028 & 1.056 & 0.706 & 0.733 & 0.889 & 4.111 & 4.222\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Hard}}\\
M1 & 53.4 & 100.0\% & 0.622 & 0.515 & 0.895 & 4.396 & 3.000 & 0.622 & 0.515 & 0.895 & 4.396 & 3.000\\
M2 & 83.9 & 93.9\% & 0.682 & 0.611 & 0.872 & 4.084 & 3.136 & 0.729 & 0.651 & 0.931 & 4.351 & 3.341\\
M3 & 98.2 & 96.8\% & 0.728 & 0.668 & 0.921 & 4.002 & 3.845 & 0.754 & 0.691 & 0.952 & 4.134 & 3.972\\
M4 & 124.0 & 93.4\% & 0.683 & 0.639 & 0.835 & 3.927 & 3.530 & 0.733 & 0.683 & 0.891 & 4.204 & 3.779\\
M5 & 473.5 & 46.1\% & 0.345 & 0.313 & 0.429 & 2.018 & 1.770 & 0.767 & 0.678 & 0.941 & 4.374 & 3.837\\
M6 & 257.1 & 98.2\% & 0.747 & 0.709 & 0.966 & 4.400 & 4.091 & 0.751 & 0.712 & 0.971 & 4.420 & 4.110\\
M7 & 1039.8 & 85.2\% & 0.676 & 0.643 & 0.907 & 4.229 & 3.677 & 0.721 & 0.684 & 0.966 & 4.495 & 3.908\\
M8 & 396.3 & 75.2\% & 0.713 & 0.652 & 0.883 & 3.818 & 3.582 & 0.738 & 0.675 & 0.915 & 3.953 & 3.708\\
M9 & 1025.1 & 83.9\% & 0.687 & 0.655 & 0.928 & 4.289 & 3.704 & 0.720 & 0.685 & 0.971 & 4.493 & 3.881\\
M10 & 600.1 & 0.0\% & 0.042 & 0.040 & 0.129 & 0.694 & 0.444 & 0.312 & 0.312 & 1.000 & 5.000 & 3.200\\
\addlinespace[2pt]
\bottomrule\end{tabular}\endgroup

==> tables/compact_results_rendering.tex <==
\begingroup\fontsize{7.2}{8.4}\selectfont\setlength{\tabcolsep}{1.6pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{@{}lrr*{10}{r}@{}}\toprule
 & & & \multicolumn{5}{c}{Auto-zero} & \multicolumn{5}{c}{Completed-only}\\
ID & 秒 & 完成率 & Dir. & Der. & Inv. & VQ & DQ & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\multicolumn{13}{l}{\textbf{HTML}}\\
M1 & 55.8 & 100.0\% & 0.703 & 0.414 & 0.944 & 4.653 & 3.580 & 0.703 & 0.414 & 0.944 & 4.653 & 3.580\\
M2 & 88.6 & 100.0\% & 0.793 & 0.604 & 0.948 & 4.595 & 3.926 & 0.793 & 0.604 & 0.948 & 4.595 & 3.926\\
M3 & 114.9 & 100.0\% & 0.768 & 0.522 & 0.979 & 4.544 & 3.966 & 0.768 & 0.522 & 0.979 & 4.544 & 3.966\\
M4 & 107.7 & 99.4\% & 0.772 & 0.519 & 0.925 & 4.671 & 3.943 & 0.777 & 0.524 & 0.931 & 4.698 & 3.966\\
M5 & 379.8 & 76.2\% & 0.600 & 0.405 & 0.703 & 3.607 & 3.148 & 0.824 & 0.568 & 0.943 & 4.731 & 4.130\\
M6 & 289.8 & 99.0\% & 0.768 & 0.544 & 0.985 & 4.698 & 4.013 & 0.768 & 0.544 & 0.985 & 4.698 & 4.013\\
M7 & 1122.7 & 86.5\% & 0.745 & 0.499 & 0.968 & 4.637 & 3.926 & 0.759 & 0.508 & 0.985 & 4.718 & 3.994\\
M8 & 425.1 & 71.1\% & 0.773 & 0.537 & 0.928 & 4.184 & 3.799 & 0.783 & 0.541 & 0.941 & 4.249 & 3.857\\
M9 & 1052.0 & 88.4\% & 0.757 & 0.519 & 0.966 & 4.663 & 3.956 & 0.767 & 0.524 & 0.980 & 4.726 & 4.010\\
M10 & 600.1 & 0.0\% & 0.139 & 0.123 & 0.330 & 1.556 & 1.222 & 0.407 & 0.364 & 0.972 & 4.667 & 3.667\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{DOT}}\\
M1 & 56.9 & 100.0\% & 0.721 & 0.632 & 0.898 & 4.240 & 3.969 & 0.721 & 0.632 & 0.898 & 4.240 & 3.969\\
M2 & 50.1 & 59.4\% & 0.478 & 0.443 & 0.580 & 2.642 & 2.576 & 0.785 & 0.704 & 0.968 & 4.449 & 4.338\\
M3 & 120.8 & 98.3\% & 0.803 & 0.724 & 0.891 & 3.852 & 3.974 & 0.827 & 0.747 & 0.911 & 3.920 & 4.044\\
M4 & 93.2 & 96.5\% & 0.771 & 0.710 & 0.815 & 3.747 & 3.664 & 0.795 & 0.733 & 0.844 & 3.882 & 3.796\\
M5 & 429.4 & 44.1\% & 0.367 & 0.329 & 0.394 & 1.847 & 1.939 & 0.832 & 0.761 & 0.910 & 4.188 & 4.396\\
M6 & 384.6 & 88.6\% & 0.812 & 0.774 & 0.913 & 4.096 & 4.175 & 0.827 & 0.790 & 0.926 & 4.150 & 4.230\\
M7 & 1366.5 & 60.3\% & 0.555 & 0.557 & 0.679 & 3.140 & 3.070 & 0.741 & 0.719 & 0.937 & 4.331 & 4.235\\
M8 & 469.2 & 48.0\% & 0.666 & 0.632 & 0.748 & 3.262 & 3.432 & 0.774 & 0.739 & 0.873 & 3.831 & 4.031\\
M9 & 1380.2 & 64.6\% & 0.607 & 0.605 & 0.740 & 3.428 & 3.376 & 0.743 & 0.731 & 0.932 & 4.386 & 4.318\\
M10 & 600.1 & 0.0\% & 0.077 & 0.091 & 0.108 & 0.667 & 0.833 & 0.667 & 1.000 & 0.667 & 4.000 & 5.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{TikZ}}\\
M1 & 52.0 & 100.0\% & 0.798 & 0.628 & 0.820 & 4.246 & 4.246 & 0.798 & 0.628 & 0.820 & 4.246 & 4.246\\
M2 & 79.9 & 100.0\% & 0.813 & 0.660 & 0.960 & 4.373 & 4.470 & 0.813 & 0.660 & 0.960 & 4.373 & 4.470\\
M3 & 96.8 & 88.1\% & 0.786 & 0.654 & 0.719 & 2.448 & 3.761 & 0.882 & 0.724 & 0.820 & 2.780 & 4.271\\
M4 & 170.4 & 85.8\% & 0.739 & 0.612 & 0.716 & 3.239 & 3.657 & 0.892 & 0.757 & 0.842 & 3.774 & 4.261\\
M5 & 536.8 & 23.9\% & 0.179 & 0.165 & 0.201 & 0.881 & 1.060 & 0.821 & 0.756 & 0.852 & 3.688 & 4.438\\
M6 & 269.5 & 98.5\% & 0.872 & 0.734 & 0.903 & 3.806 & 4.508 & 0.875 & 0.734 & 0.908 & 3.835 & 4.541\\
M7 & 1244.8 & 67.2\% & 0.728 & 0.601 & 0.785 & 3.724 & 3.910 & 0.827 & 0.689 & 0.913 & 4.265 & 4.479\\
M8 & 460.3 & 58.2\% & 0.802 & 0.702 & 0.794 & 3.351 & 3.955 & 0.831 & 0.725 & 0.825 & 3.508 & 4.141\\
M9 & 1368.6 & 61.9\% & 0.685 & 0.564 & 0.775 & 3.590 & 3.791 & 0.800 & 0.675 & 0.897 & 4.111 & 4.342\\
M10 & 600.1 & 0.0\% & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{CircuitikZ}}\\
M1 & 44.4 & 100.0\% & 0.720 & 0.659 & 0.952 & 4.385 & 3.975 & 0.720 & 0.659 & 0.952 & 4.385 & 3.975\\
M2 & 72.5 & 100.0\% & 0.781 & 0.731 & 0.963 & 4.435 & 4.062 & 0.781 & 0.731 & 0.963 & 4.435 & 4.062\\
M3 & 73.7 & 90.7\% & 0.695 & 0.659 & 0.837 & 3.106 & 3.689 & 0.774 & 0.742 & 0.927 & 3.425 & 4.069\\
M4 & 181.9 & 84.5\% & 0.649 & 0.560 & 0.743 & 3.410 & 3.280 & 0.786 & 0.698 & 0.894 & 4.037 & 3.882\\
M5 & 548.3 & 18.0\% & 0.141 & 0.121 & 0.160 & 0.814 & 0.758 & 0.815 & 0.730 & 0.961 & 4.517 & 4.207\\
M6 & 200.8 & 95.0\% & 0.781 & 0.771 & 0.925 & 4.118 & 4.143 & 0.805 & 0.785 & 0.959 & 4.305 & 4.331\\
M7 & 950.2 & 87.6\% & 0.727 & 0.686 & 0.905 & 4.168 & 4.106 & 0.774 & 0.725 & 0.958 & 4.415 & 4.349\\
M8 & 430.3 & 66.5\% & 0.704 & 0.682 & 0.873 & 3.404 & 3.584 & 0.718 & 0.697 & 0.894 & 3.490 & 3.675\\
M9 & 1083.3 & 80.1\% & 0.720 & 0.668 & 0.877 & 3.907 & 3.708 & 0.786 & 0.720 & 0.961 & 4.308 & 4.089\\
M10 & 600.1 & 0.0\% & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\addlinespace[2pt]
\multicolumn{13}{l}{\textbf{Python}}\\
M1 & 46.6 & 100.0\% & 0.749 & 0.539 & 0.908 & 4.466 & 3.746 & 0.749 & 0.539 & 0.908 & 4.466 & 3.746\\
M2 & 73.4 & 99.6\% & 0.819 & 0.684 & 0.934 & 4.361 & 3.979 & 0.826 & 0.691 & 0.938 & 4.378 & 3.994\\
M3 & 84.9 & 98.3\% & 0.888 & 0.795 & 0.958 & 4.361 & 4.497 & 0.906 & 0.809 & 0.974 & 4.438 & 4.576\\
M4 & 107.2 & 94.5\% & 0.836 & 0.744 & 0.782 & 3.774 & 3.931 & 0.890 & 0.787 & 0.830 & 3.996 & 4.162\\
M5 & 479.0 & 44.0\% & 0.379 & 0.324 & 0.385 & 1.830 & 1.883 & 0.909 & 0.779 & 0.886 & 4.161 & 4.283\\
M6 & 221.9 & 98.7\% & 0.893 & 0.804 & 0.970 & 4.566 & 4.579 & 0.901 & 0.810 & 0.982 & 4.619 & 4.633\\
M7 & 917.1 & 90.8\% & 0.884 & 0.797 & 0.959 & 4.575 & 4.543 & 0.894 & 0.805 & 0.974 & 4.647 & 4.614\\
M8 & 427.1 & 69.4\% & 0.824 & 0.712 & 0.840 & 3.772 & 3.851 & 0.868 & 0.739 & 0.887 & 3.986 & 4.069\\
M9 & 968.9 & 84.1\% & 0.880 & 0.783 & 0.976 & 4.616 & 4.501 & 0.889 & 0.790 & 0.986 & 4.660 & 4.544\\
M10 & 580.2 & 13.9\% & 0.186 & 0.109 & 0.248 & 1.306 & 1.222 & 0.929 & 0.750 & 1.000 & 4.700 & 4.400\\
\addlinespace[2pt]
\bottomrule\end{tabular}\endgroup

==> tables/composition.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrrrrr}
\caption{VAO-Bench 及其消融子集 VAC-Bench-Ablation 的组成。源数按源产物去重。}\label{tab:app-composition}\\
\toprule
类别 & 渲染 & 源数 & Easy & Medium & Hard & 主集 & 子集\\\midrule
\endfirsthead
\toprule
类别 & 渲染 & 源数 & Easy & Medium & Hard & 主集 & 子集\\\midrule
\endhead
\bottomrule\endfoot
商业网页 & HTML & 160 & 73 & 67 & 56 & 196 & 40\\
科研文档 & HTML & 112 & 49 & 45 & 45 & 139 & 28\\
交互数据面板 & HTML & 154 & 71 & 62 & 58 & 191 & 38\\
流程与工作流 & DOT & 187 & 87 & 78 & 64 & 229 & 46\\
系统与架构 & TikZ & 107 & 55 & 45 & 34 & 134 & 26\\
电路与逻辑 & CircuitikZ & 138 & 68 & 55 & 38 & 161 & 33\\
科研统计图 & Python & 126 & 55 & 50 & 46 & 151 & 31\\
数学与几何 & Python & 135 & 64 & 57 & 46 & 167 & 34\\
化学分子图 & Python & 177 & 78 & 74 & 53 & 205 & 40\\
合计 &  & 1296 & 600 & 533 & 440 & 1573 & 316\\
\end{longtable}\endgroup


==> tables/coverage.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{lrrrrrrr}
\caption{运行覆盖审计。恢复数是超时记录的子集，不能与超时数相加；其他失败包括模型、代码和渲染错误。缺失任务不自动计零。}\label{tab:app-coverage}\\
\toprule
方法 & 汇总分母 & 缺记录 & 正常 & 恢复 & 超时 & 其他失败 & 设施异常\\\midrule
\endfirsthead
\toprule
方法 & 汇总分母 & 缺记录 & 正常 & 恢复 & 超时 & 其他失败 & 设施异常\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & 1571 & 2 & 1571 & 0 & 0 & 0 & 0\\
Seedream-5.0-Pro & 1573 & 0 & 1478 & 0 & 0 & 95 & 0\\
GPT-5.6-Sol & 1573 & 0 & 1529 & 0 & 0 & 44 & 0\\
DeepSeek-Flash & 1573 & 0 & 1489 & 0 & 0 & 84 & 0\\
GLM-5.3-Flash & 1573 & 0 & 793 & 0 & 774 & 6 & 0\\
Codex-GPT & 1573 & 0 & 1525 & 31 & 33 & 15 & 0\\
Codex-DeepSeek & 1573 & 0 & 1299 & 168 & 248 & 26 & 0\\
Codex-GLM & 1573 & 0 & 1032 & 461 & 519 & 22 & 0\\
CC-DeepSeek & 1573 & 0 & 1265 & 214 & 281 & 27 & 0\\
CC-GLM & 108 & 1465 & 5 & 19 & 103 & 0 & 0\\
\end{longtable}\endgroup


==> tables/denominators.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr}
\caption{总体评分点分母。失败计零对应 auto-zero，仅成功评分对应 completed-only；两者均纳入超时恢复后成功评分的产物。}\label{tab:app-denominators}\\
\toprule
方法 & 统计口径 & Direct & Derived & Invariant\\\midrule
\endfirsthead
\toprule
方法 & 统计口径 & Direct & Derived & Invariant\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & 失败计零 & 3148 & 2410 & 4769\\
GPT-Image-2 & 仅成功评分 & 3148 & 2410 & 4769\\
Seedream-5.0-Pro & 失败计零 & 3154 & 2416 & 4775\\
Seedream-5.0-Pro & 仅成功评分 & 2967 & 2275 & 4477\\
GPT-5.6-Sol & 失败计零 & 3154 & 2416 & 4775\\
GPT-5.6-Sol & 仅成功评分 & 3060 & 2348 & 4643\\
DeepSeek-Flash & 失败计零 & 3154 & 2416 & 4775\\
DeepSeek-Flash & 仅成功评分 & 2972 & 2273 & 4514\\
GLM-5.3-Flash & 失败计零 & 3154 & 2416 & 4775\\
GLM-5.3-Flash & 仅成功评分 & 1542 & 1174 & 2377\\
Codex-GPT & 失败计零 & 3154 & 2416 & 4775\\
Codex-GPT & 仅成功评分 & 3126 & 2399 & 4728\\
Codex-DeepSeek & 失败计零 & 3154 & 2416 & 4775\\
Codex-DeepSeek & 仅成功评分 & 2956 & 2275 & 4446\\
Codex-GLM & 失败计零 & 3154 & 2416 & 4775\\
Codex-GLM & 仅成功评分 & 3009 & 2317 & 4539\\
CC-DeepSeek & 失败计零 & 3154 & 2416 & 4775\\
CC-DeepSeek & 仅成功评分 & 2983 & 2291 & 4495\\
CC-GLM & 失败计零 & 231 & 182 & 330\\
CC-GLM & 仅成功评分 & 44 & 32 & 70\\
\end{longtable}\endgroup


==> tables/domain_scores_1.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分示例：商业网页。}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 1/1 & -- & 2/2 & 5 & 3\\
Seedream-5.0-Pro & 1/1 & -- & 2/2 & 5 & 5\\
GPT-5.6-Sol & 1/1 & -- & 2/2 & 5 & 5\\
DeepSeek-Flash & 1/1 & -- & 2/2 & 5 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_2.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：科研文档。}\label{tab:app-domain-example-2}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 2/2 & 1/2 & 3/3 & 4 & 3\\
DeepSeek-Flash & 2/2 & 1/2 & 3/3 & 4 & 3\\
Codex-GPT & 2/2 & 2/2 & 3/3 & 4 & 3\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_3.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：交互数据面板。}\label{tab:app-domain-example-3}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 2/4 & 4/4 & 3/3 & 5 & 3\\
DeepSeek-Flash & 4/4 & 4/4 & 3/3 & 4 & 5\\
Codex-GPT & 4/4 & 4/4 & 3/3 & 5 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_4.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：流程与工作流。}\label{tab:app-domain-example-4}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 1/1 & -- & 3/3 & 4 & 5\\
DeepSeek-Flash & 1/1 & -- & 1/3 & 4 & 3\\
Codex-GPT & 1/1 & -- & 3/3 & 4 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_5.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：系统与架构。}\label{tab:app-domain-example-5}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 1/1 & -- & 3/3 & 4 & 5\\
DeepSeek-Flash & 1/1 & -- & 1/3 & 3 & 4\\
Codex-GPT & 1/1 & -- & 1/3 & 3 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_6.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：电路与逻辑。}\label{tab:app-domain-example-6}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 1/1 & -- & 2/2 & 4 & 5\\
DeepSeek-Flash & 1/1 & -- & 2/2 & 5 & 5\\
Codex-GPT & 1/1 & -- & 2/2 & 5 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_7.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：科研统计图。}\label{tab:app-domain-example-7}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 1/1 & -- & 3/3 & 5 & 5\\
DeepSeek-Flash & 1/1 & -- & 3/3 & 5 & 5\\
Codex-GPT & 1/1 & -- & 3/3 & 5 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_8.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：数学与几何。}\label{tab:app-domain-example-8}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 0/1 & -- & 2/2 & 3 & 3\\
DeepSeek-Flash & 1/1 & -- & 2/2 & 4 & 4\\
Codex-GPT & 1/1 & -- & 2/2 & 5 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/domain_scores_9.tex <==
\begin{table}[h]\centering\footnotesize
\caption{同题输出的逐项评分：化学分子图。}\label{tab:app-domain-example-9}
\begin{tabular}{lrrrrr}\toprule
方法 & Direct & Derived & Invariant & VQ & DQ\\\midrule
GPT-Image-2 & 1/1 & -- & 3/3 & 5 & 5\\
DeepSeek-Flash & 1/1 & -- & 2/3 & 5 & 2\\
Codex-GPT & 1/1 & -- & 3/3 & 5 & 5\\
\bottomrule\end{tabular}\end{table}


==> tables/operations.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{p{0.70\linewidth}rr}
\caption{VAO-Bench 的 14 种操作及任务数量。}\label{tab:app-operations}\\
\toprule
操作类型 & 难度 & 任务数\\\midrule
\endfirsthead
\toprule
操作类型 & 难度 & 任务数\\\midrule
\endhead
\bottomrule\endfoot
标签与文本重命名 & Easy & 200\\
颜色、样式、标记与徽标修改 & Easy & 128\\
注释、图注与图例修改 & Easy & 149\\
高亮、状态与选择修改 & Easy & 123\\
局部数值更新与视觉同步 & Medium & 178\\
局部组件增删、重连与重排 & Medium & 114\\
面板、节点或对象组移动重排 & Medium & 90\\
派生标签、摘要与引用更新 & Medium & 97\\
局部分组编码与样式同步 & Medium & 54\\
全局阈值、筛选与基线传播 & Hard & 98\\
含依赖关系的结构重构 & Hard & 106\\
派生指标、几何、逻辑与化学关系重算 & Hard & 128\\
多面板与多区域布局变换 & Hard & 54\\
领域一致性修复 & Hard & 54\\
\end{longtable}\endgroup


==> tables/points.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{lrrrrr}
\caption{评分点总数 / 每题均值；最后一列为不含 Derived 点的任务数。}\label{tab:app-points}\\
\toprule
难度 & 任务数 & Direct & Derived & Invariant & 无派生点\\\midrule
\endfirsthead
\toprule
难度 & 任务数 & Direct & Derived & Invariant & 无派生点\\\midrule
\endhead
\bottomrule\endfoot
Easy & 600 & 691 / 1.15 & 9 / 0.01 & 1546 / 2.58 & 592\\
Medium & 533 & 995 / 1.87 & 884 / 1.66 & 1594 / 2.99 & 0\\
Hard & 440 & 1468 / 3.34 & 1523 / 3.46 & 1635 / 3.72 & 0\\
\end{longtable}\endgroup


==> tables/result_difficulty_easy.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{难度分组：Easy。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-difficulty-0}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 600/600 & 600/600 & 50.1 & 0.8973 & 0.5556 & 0.9288 & 4.5700 & 4.5200\\
GPT-Image-2 & CO & 600/600 & 600/600 & 50.1 & 0.8973 & 0.5556 & 0.9288 & 4.5700 & 4.5200\\
Seedream-5.0-Pro & AZ & 560/600 & 560/600 & 70.0 & 0.8842 & 0.6667 & 0.8997 & 4.3000 & 4.3383\\
Seedream-5.0-Pro & CO & 560/600 & 560/600 & 70.0 & 0.9386 & 0.6667 & 0.9673 & 4.6071 & 4.6482\\
GPT-5.6-Sol & AZ & 582/600 & 582/600 & 102.4 & 0.9161 & 0.5556 & 0.9198 & 4.1150 & 4.3683\\
GPT-5.6-Sol & CO & 582/600 & 582/600 & 102.4 & 0.9434 & 0.5556 & 0.9461 & 4.2423 & 4.5034\\
DeepSeek-Flash & AZ & 572/600 & 572/600 & 113.1 & 0.9088 & 0.5556 & 0.8105 & 4.0267 & 4.0967\\
DeepSeek-Flash & CO & 572/600 & 572/600 & 113.1 & 0.9544 & 0.6250 & 0.8524 & 4.2238 & 4.2972\\
GLM-5.3-Flash & AZ & 312/600 & 312/600 & 434.9 & 0.5007 & 0.5556 & 0.4573 & 2.3267 & 2.3633\\
GLM-5.3-Flash & CO & 312/600 & 312/600 & 434.9 & 0.9584 & 1.0000 & 0.8893 & 4.4744 & 4.5449\\
Codex-GPT & AZ & 572/600 & 592/600 & 282.7 & 0.9334 & 0.6667 & 0.9457 & 4.4800 & 4.5917\\
Codex-GPT & CO & 572/600 & 592/600 & 282.7 & 0.9444 & 0.6667 & 0.9574 & 4.5405 & 4.6537\\
Codex-DeepSeek & AZ & 475/600 & 550/600 & 1125.4 & 0.8495 & 0.6667 & 0.8784 & 4.2933 & 4.3083\\
Codex-DeepSeek & CO & 475/600 & 550/600 & 1125.4 & 0.9172 & 0.6667 & 0.9618 & 4.6836 & 4.7000\\
Codex-GLM & AZ & 341/600 & 562/600 & 463.4 & 0.8625 & 0.6667 & 0.8111 & 3.7517 & 3.9967\\
Codex-GLM & CO & 341/600 & 562/600 & 463.4 & 0.9198 & 0.6667 & 0.8672 & 4.0053 & 4.2669\\
CC-DeepSeek & AZ & 459/600 & 562/600 & 1161.3 & 0.8770 & 0.6667 & 0.9004 & 4.3450 & 4.3717\\
CC-DeepSeek & CO & 459/600 & 562/600 & 1161.3 & 0.9309 & 0.6667 & 0.9627 & 4.6388 & 4.6673\\
CC-GLM & AZ & 2/36 & 10/36 & 586.9 & 0.2093 & 0.0000 & 0.2857 & 1.3611 & 1.2222\\
CC-GLM & CO & 2/36 & 10/36 & 586.9 & 0.8182 & 0.0000 & 1.0000 & 4.9000 & 4.4000\\
\end{longtable}\endgroup


==> tables/result_difficulty_hard.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{难度分组：Hard。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-difficulty-2}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 440/440 & 440/440 & 53.4 & 0.6223 & 0.5148 & 0.8952 & 4.3964 & 3.0000\\
GPT-Image-2 & CO & 440/440 & 440/440 & 53.4 & 0.6223 & 0.5148 & 0.8952 & 4.3964 & 3.0000\\
Seedream-5.0-Pro & AZ & 413/440 & 413/440 & 83.9 & 0.6819 & 0.6113 & 0.8716 & 4.0841 & 3.1364\\
Seedream-5.0-Pro & CO & 413/440 & 413/440 & 83.9 & 0.7291 & 0.6510 & 0.9308 & 4.3511 & 3.3414\\
GPT-5.6-Sol & AZ & 426/440 & 426/440 & 98.2 & 0.7275 & 0.6684 & 0.9211 & 4.0023 & 3.8455\\
GPT-5.6-Sol & CO & 426/440 & 426/440 & 98.2 & 0.7537 & 0.6911 & 0.9520 & 4.1338 & 3.9718\\
DeepSeek-Flash & AZ & 411/440 & 411/440 & 124.0 & 0.6832 & 0.6389 & 0.8349 & 3.9273 & 3.5295\\
DeepSeek-Flash & CO & 411/440 & 411/440 & 124.0 & 0.7327 & 0.6828 & 0.8910 & 4.2044 & 3.7786\\
GLM-5.3-Flash & AZ & 203/440 & 203/440 & 473.5 & 0.3454 & 0.3132 & 0.4287 & 2.0182 & 1.7705\\
GLM-5.3-Flash & CO & 203/440 & 203/440 & 473.5 & 0.7670 & 0.6785 & 0.9409 & 4.3744 & 3.8374\\
Codex-GPT & AZ & 432/440 & 438/440 & 257.1 & 0.7473 & 0.7091 & 0.9664 & 4.4000 & 4.0909\\
Codex-GPT & CO & 432/440 & 438/440 & 257.1 & 0.7509 & 0.7124 & 0.9711 & 4.4201 & 4.1096\\
Codex-DeepSeek & AZ & 375/440 & 414/440 & 1039.8 & 0.6764 & 0.6435 & 0.9070 & 4.2295 & 3.6773\\
Codex-DeepSeek & CO & 375/440 & 414/440 & 1039.8 & 0.7211 & 0.6844 & 0.9661 & 4.4952 & 3.9082\\
Codex-GLM & AZ & 331/440 & 425/440 & 396.3 & 0.7125 & 0.6520 & 0.8826 & 3.8182 & 3.5818\\
Codex-GLM & CO & 331/440 & 425/440 & 396.3 & 0.7382 & 0.6751 & 0.9150 & 3.9529 & 3.7082\\
CC-DeepSeek & AZ & 369/440 & 420/440 & 1025.1 & 0.6873 & 0.6546 & 0.9284 & 4.2886 & 3.7045\\
CC-DeepSeek & CO & 369/440 & 420/440 & 1025.1 & 0.7202 & 0.6852 & 0.9712 & 4.4929 & 3.8810\\
CC-GLM & AZ & 0/36 & 5/36 & 600.1 & 0.0420 & 0.0397 & 0.1288 & 0.6944 & 0.4444\\
CC-GLM & CO & 0/36 & 5/36 & 600.1 & 0.3125 & 0.3125 & 1.0000 & 5.0000 & 3.2000\\
\end{longtable}\endgroup


==> tables/result_difficulty_middle.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{难度分组：Medium。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-difficulty-1}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 533/533 & 533/533 & 51.1 & 0.7724 & 0.5465 & 0.9252 & 4.4135 & 3.6165\\
GPT-Image-2 & CO & 533/533 & 533/533 & 51.1 & 0.7724 & 0.5465 & 0.9252 & 4.4135 & 3.6165\\
Seedream-5.0-Pro & AZ & 505/533 & 505/533 & 74.9 & 0.7769 & 0.6403 & 0.8984 & 4.1764 & 3.7636\\
Seedream-5.0-Pro & CO & 505/533 & 505/533 & 74.9 & 0.8197 & 0.6770 & 0.9496 & 4.4079 & 3.9723\\
GPT-5.6-Sol & AZ & 521/533 & 521/533 & 98.9 & 0.8462 & 0.6561 & 0.9329 & 4.0356 & 4.0019\\
GPT-5.6-Sol & CO & 521/533 & 521/533 & 98.9 & 0.8663 & 0.6697 & 0.9544 & 4.1286 & 4.0940\\
DeepSeek-Flash & AZ & 506/533 & 506/533 & 119.6 & 0.8261 & 0.6188 & 0.8331 & 3.9925 & 3.7073\\
DeepSeek-Flash & CO & 506/533 & 506/533 & 119.6 & 0.8698 & 0.6512 & 0.8783 & 4.2055 & 3.9051\\
GLM-5.3-Flash & AZ & 278/533 & 278/533 & 449.4 & 0.4573 & 0.3360 & 0.4875 & 2.3302 & 2.1614\\
GLM-5.3-Flash & CO & 278/533 & 278/533 & 449.4 & 0.8750 & 0.6373 & 0.9283 & 4.4676 & 4.1439\\
Codex-GPT & AZ & 521/533 & 526/533 & 267.0 & 0.8633 & 0.6799 & 0.9586 & 4.4015 & 4.0863\\
Codex-GPT & CO & 521/533 & 526/533 & 267.0 & 0.8747 & 0.6876 & 0.9708 & 4.4601 & 4.1407\\
Codex-DeepSeek & AZ & 449/533 & 503/533 & 1069.6 & 0.8181 & 0.6052 & 0.9159 & 4.2852 & 3.9887\\
Codex-DeepSeek & CO & 449/533 & 503/533 & 1069.6 & 0.8669 & 0.6415 & 0.9740 & 4.5408 & 4.2266\\
Codex-GLM & AZ & 360/533 & 506/533 & 437.0 & 0.7889 & 0.6029 & 0.8695 & 3.7280 & 3.6229\\
Codex-GLM & CO & 360/533 & 506/533 & 437.0 & 0.8316 & 0.6368 & 0.9142 & 3.9269 & 3.8162\\
CC-DeepSeek & AZ & 437/533 & 497/533 & 1099.7 & 0.8040 & 0.5995 & 0.9053 & 4.2552 & 3.8649\\
CC-DeepSeek & CO & 437/533 & 497/533 & 1099.7 & 0.8593 & 0.6409 & 0.9711 & 4.5634 & 4.1449\\
CC-GLM & AZ & 3/36 & 9/36 & 593.4 & 0.1739 & 0.2000 & 0.2243 & 1.0278 & 1.0556\\
CC-GLM & CO & 3/36 & 9/36 & 593.4 & 0.7059 & 0.7333 & 0.8889 & 4.1111 & 4.2222\\
\end{longtable}\endgroup


==> tables/result_domain_Business_Web_Interfaces.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：商业网页。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-0}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 196/196 & 196/196 & 55.4 & 0.6886 & 0.3710 & 0.9509 & 4.8214 & 3.7398\\
GPT-Image-2 & CO & 196/196 & 196/196 & 55.4 & 0.6886 & 0.3710 & 0.9509 & 4.8214 & 3.7398\\
Seedream-5.0-Pro & AZ & 196/196 & 196/196 & 88.9 & 0.8101 & 0.5903 & 0.9442 & 4.7704 & 4.0102\\
Seedream-5.0-Pro & CO & 196/196 & 196/196 & 88.9 & 0.8101 & 0.5903 & 0.9442 & 4.7704 & 4.0102\\
GPT-5.6-Sol & AZ & 196/196 & 196/196 & 119.6 & 0.7848 & 0.4484 & 0.9712 & 4.6888 & 4.0051\\
GPT-5.6-Sol & CO & 196/196 & 196/196 & 119.6 & 0.7848 & 0.4484 & 0.9712 & 4.6888 & 4.0051\\
DeepSeek-Flash & AZ & 194/196 & 194/196 & 91.9 & 0.7949 & 0.4452 & 0.9323 & 4.7398 & 3.9745\\
DeepSeek-Flash & CO & 194/196 & 194/196 & 91.9 & 0.8051 & 0.4539 & 0.9435 & 4.7887 & 4.0155\\
GLM-5.3-Flash & AZ & 164/196 & 164/196 & 368.8 & 0.6405 & 0.3452 & 0.7597 & 4.0357 & 3.4541\\
GLM-5.3-Flash & CO & 164/196 & 164/196 & 368.8 & 0.8161 & 0.4553 & 0.9354 & 4.8232 & 4.1280\\
Codex-GPT & AZ & 196/196 & 196/196 & 274.6 & 0.7696 & 0.4645 & 0.9780 & 4.8520 & 4.0255\\
Codex-GPT & CO & 196/196 & 196/196 & 274.6 & 0.7696 & 0.4645 & 0.9780 & 4.8520 & 4.0255\\
Codex-DeepSeek & AZ & 187/196 & 195/196 & 1018.6 & 0.7519 & 0.4452 & 0.9780 & 4.8163 & 4.0255\\
Codex-DeepSeek & CO & 187/196 & 195/196 & 1018.6 & 0.7538 & 0.4452 & 0.9813 & 4.8410 & 4.0462\\
Codex-GLM & AZ & 163/196 & 196/196 & 388.6 & 0.7646 & 0.4419 & 0.9492 & 4.3827 & 3.8061\\
Codex-GLM & CO & 163/196 & 196/196 & 388.6 & 0.7646 & 0.4419 & 0.9492 & 4.3827 & 3.8061\\
CC-DeepSeek & AZ & 193/196 & 196/196 & 876.6 & 0.7797 & 0.4710 & 0.9797 & 4.8571 & 4.0510\\
CC-DeepSeek & CO & 193/196 & 196/196 & 876.6 & 0.7797 & 0.4710 & 0.9797 & 4.8571 & 4.0510\\
CC-GLM & AZ & 0/12 & 5/12 & 600.1 & 0.2400 & 0.1429 & 0.3714 & 2.0833 & 1.5833\\
CC-GLM & CO & 0/12 & 5/12 & 600.1 & 0.6000 & 0.3750 & 0.9286 & 5.0000 & 3.8000\\
\end{longtable}\endgroup


==> tables/result_domain_Chemistry_and_Molecular_Figures.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：化学分子图。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-1}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 205/205 & 205/205 & 40.1 & 0.7704 & 0.7063 & 0.9028 & 4.7854 & 4.2780\\
GPT-Image-2 & CO & 205/205 & 205/205 & 40.1 & 0.7704 & 0.7063 & 0.9028 & 4.7854 & 4.2780\\
Seedream-5.0-Pro & AZ & 203/205 & 203/205 & 66.4 & 0.8087 & 0.7517 & 0.9275 & 4.5659 & 4.2585\\
Seedream-5.0-Pro & CO & 203/205 & 203/205 & 66.4 & 0.8255 & 0.7734 & 0.9391 & 4.6108 & 4.3005\\
GPT-5.6-Sol & AZ & 204/205 & 204/205 & 72.1 & 0.8495 & 0.7517 & 0.9537 & 4.6878 & 4.4878\\
GPT-5.6-Sol & CO & 204/205 & 204/205 & 72.1 & 0.8538 & 0.7517 & 0.9581 & 4.7108 & 4.5098\\
DeepSeek-Flash & AZ & 185/205 & 185/205 & 114.5 & 0.7449 & 0.6364 & 0.6497 & 3.6683 & 3.6146\\
DeepSeek-Flash & CO & 185/205 & 185/205 & 114.5 & 0.8391 & 0.7109 & 0.7221 & 4.0649 & 4.0054\\
GLM-5.3-Flash & AZ & 77/205 & 77/205 & 496.7 & 0.3061 & 0.2797 & 0.2917 & 1.5317 & 1.5659\\
GLM-5.3-Flash & CO & 77/205 & 77/205 & 496.7 & 0.8451 & 0.7477 & 0.7842 & 4.0779 & 4.1688\\
Codex-GPT & AZ & 200/205 & 200/205 & 176.1 & 0.8214 & 0.7552 & 0.9506 & 4.7073 & 4.5610\\
Codex-GPT & CO & 200/205 & 200/205 & 176.1 & 0.8385 & 0.7687 & 0.9747 & 4.8250 & 4.6750\\
Codex-DeepSeek & AZ & 184/205 & 200/205 & 801.0 & 0.8265 & 0.7343 & 0.9414 & 4.6439 & 4.5171\\
Codex-DeepSeek & CO & 184/205 & 200/205 & 801.0 & 0.8394 & 0.7394 & 0.9637 & 4.7600 & 4.6300\\
Codex-GLM & AZ & 138/205 & 186/205 & 438.8 & 0.7653 & 0.6678 & 0.7840 & 3.9707 & 3.7951\\
Codex-GLM & CO & 138/205 & 186/205 & 438.8 & 0.8333 & 0.7074 & 0.8552 & 4.3763 & 4.1828\\
CC-DeepSeek & AZ & 186/205 & 202/205 & 793.9 & 0.8418 & 0.7448 & 0.9660 & 4.7366 & 4.4732\\
CC-DeepSeek & CO & 186/205 & 202/205 & 793.9 & 0.8505 & 0.7527 & 0.9812 & 4.8069 & 4.5396\\
CC-GLM & AZ & 5/12 & 6/12 & 540.4 & 0.3182 & 0.1429 & 0.4571 & 2.4167 & 2.1667\\
CC-GLM & CO & 5/12 & 6/12 & 540.4 & 0.8750 & 0.5000 & 1.0000 & 4.8333 & 4.3333\\
\end{longtable}\endgroup


==> tables/result_domain_Circuit_and_Logic_Diagrams.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：电路与逻辑。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-2}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 161/161 & 161/161 & 44.4 & 0.7203 & 0.6592 & 0.9516 & 4.3851 & 3.9752\\
GPT-Image-2 & CO & 161/161 & 161/161 & 44.4 & 0.7203 & 0.6592 & 0.9516 & 4.3851 & 3.9752\\
Seedream-5.0-Pro & AZ & 161/161 & 161/161 & 72.5 & 0.7814 & 0.7309 & 0.9626 & 4.4348 & 4.0621\\
Seedream-5.0-Pro & CO & 161/161 & 161/161 & 72.5 & 0.7814 & 0.7309 & 0.9626 & 4.4348 & 4.0621\\
GPT-5.6-Sol & AZ & 146/161 & 146/161 & 73.7 & 0.6945 & 0.6592 & 0.8374 & 3.1056 & 3.6894\\
GPT-5.6-Sol & CO & 146/161 & 146/161 & 73.7 & 0.7742 & 0.7424 & 0.9270 & 3.4247 & 4.0685\\
DeepSeek-Flash & AZ & 136/161 & 136/161 & 181.9 & 0.6495 & 0.5605 & 0.7429 & 3.4099 & 3.2795\\
DeepSeek-Flash & CO & 136/161 & 136/161 & 181.9 & 0.7860 & 0.6983 & 0.8942 & 4.0368 & 3.8824\\
GLM-5.3-Flash & AZ & 29/161 & 29/161 & 548.3 & 0.1415 & 0.1211 & 0.1604 & 0.8137 & 0.7578\\
GLM-5.3-Flash & CO & 29/161 & 29/161 & 548.3 & 0.8148 & 0.7297 & 0.9605 & 4.5172 & 4.2069\\
Codex-GPT & AZ & 153/161 & 154/161 & 200.8 & 0.7814 & 0.7713 & 0.9253 & 4.1180 & 4.1429\\
Codex-GPT & CO & 153/161 & 154/161 & 200.8 & 0.8046 & 0.7854 & 0.9590 & 4.3052 & 4.3312\\
Codex-DeepSeek & AZ & 141/161 & 152/161 & 950.2 & 0.7267 & 0.6861 & 0.9055 & 4.1677 & 4.1056\\
Codex-DeepSeek & CO & 141/161 & 152/161 & 950.2 & 0.7740 & 0.7251 & 0.9581 & 4.4145 & 4.3487\\
Codex-GLM & AZ & 107/161 & 157/161 & 430.3 & 0.7042 & 0.6816 & 0.8725 & 3.4037 & 3.5839\\
Codex-GLM & CO & 107/161 & 157/161 & 430.3 & 0.7180 & 0.6972 & 0.8941 & 3.4904 & 3.6752\\
CC-DeepSeek & AZ & 129/161 & 146/161 & 1083.3 & 0.7203 & 0.6682 & 0.8769 & 3.9068 & 3.7081\\
CC-DeepSeek & CO & 129/161 & 146/161 & 1083.3 & 0.7860 & 0.7198 & 0.9614 & 4.3082 & 4.0890\\
CC-GLM & AZ & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
CC-GLM & CO & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
\end{longtable}\endgroup


==> tables/result_domain_Interactive_Data_Panels.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：交互数据面板。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-3}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 191/191 & 191/191 & 53.5 & 0.7020 & 0.3810 & 0.9561 & 4.6508 & 3.4127\\
GPT-Image-2 & CO & 191/191 & 191/191 & 53.5 & 0.7020 & 0.3810 & 0.9561 & 4.6508 & 3.4127\\
Seedream-5.0-Pro & AZ & 191/191 & 191/191 & 86.7 & 0.8083 & 0.5701 & 0.9583 & 4.6073 & 3.8168\\
Seedream-5.0-Pro & CO & 191/191 & 191/191 & 86.7 & 0.8083 & 0.5701 & 0.9583 & 4.6073 & 3.8168\\
GPT-5.6-Sol & AZ & 191/191 & 191/191 & 112.6 & 0.7403 & 0.4922 & 0.9861 & 4.5393 & 3.8691\\
GPT-5.6-Sol & CO & 191/191 & 191/191 & 112.6 & 0.7403 & 0.4922 & 0.9861 & 4.5393 & 3.8691\\
DeepSeek-Flash & AZ & 191/191 & 191/191 & 114.0 & 0.7427 & 0.4953 & 0.9287 & 4.7225 & 3.8848\\
DeepSeek-Flash & CO & 191/191 & 191/191 & 114.0 & 0.7427 & 0.4953 & 0.9287 & 4.7225 & 3.8848\\
GLM-5.3-Flash & AZ & 147/191 & 147/191 & 362.4 & 0.6214 & 0.4548 & 0.7183 & 3.6178 & 3.2042\\
GLM-5.3-Flash & CO & 147/191 & 147/191 & 362.4 & 0.8366 & 0.6083 & 0.9408 & 4.7007 & 4.1633\\
Codex-GPT & AZ & 187/191 & 191/191 & 300.5 & 0.7354 & 0.5171 & 0.9913 & 4.6387 & 3.9791\\
Codex-GPT & CO & 187/191 & 191/191 & 300.5 & 0.7354 & 0.5171 & 0.9913 & 4.6387 & 3.9791\\
Codex-DeepSeek & AZ & 182/191 & 189/191 & 992.5 & 0.7379 & 0.5047 & 0.9774 & 4.6702 & 3.8953\\
Codex-DeepSeek & CO & 182/191 & 189/191 & 992.5 & 0.7451 & 0.5062 & 0.9894 & 4.7196 & 3.9365\\
Codex-GLM & AZ & 125/191 & 189/191 & 442.8 & 0.7985 & 0.5950 & 0.9287 & 4.2251 & 3.9267\\
Codex-GLM & CO & 125/191 & 189/191 & 442.8 & 0.8044 & 0.5950 & 0.9368 & 4.2698 & 3.9683\\
CC-DeepSeek & AZ & 180/191 & 191/191 & 968.0 & 0.7451 & 0.5047 & 0.9861 & 4.7016 & 3.9162\\
CC-DeepSeek & CO & 180/191 & 191/191 & 968.0 & 0.7451 & 0.5047 & 0.9861 & 4.7016 & 3.9162\\
CC-GLM & AZ & 0/12 & 5/12 & 600.1 & 0.1481 & 0.1739 & 0.4571 & 2.0000 & 1.5000\\
CC-GLM & CO & 0/12 & 5/12 & 600.1 & 0.3077 & 0.3636 & 1.0000 & 4.8000 & 3.6000\\
\end{longtable}\endgroup


==> tables/result_domain_Mathematical_and_Geometric_Figures.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：数学与几何。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-4}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 167/167 & 167/167 & 46.3 & 0.6636 & 0.3900 & 0.8775 & 4.2635 & 3.3593\\
GPT-Image-2 & CO & 167/167 & 167/167 & 46.3 & 0.6636 & 0.3900 & 0.8775 & 4.2635 & 3.3593\\
Seedream-5.0-Pro & AZ & 167/167 & 167/167 & 72.8 & 0.7939 & 0.6409 & 0.9116 & 4.1737 & 3.7006\\
Seedream-5.0-Pro & CO & 167/167 & 167/167 & 72.8 & 0.7939 & 0.6409 & 0.9116 & 4.1737 & 3.7006\\
GPT-5.6-Sol & AZ & 160/167 & 160/167 & 92.4 & 0.9182 & 0.8958 & 0.9418 & 4.2455 & 4.6766\\
GPT-5.6-Sol & CO & 160/167 & 160/167 & 92.4 & 0.9650 & 0.9317 & 0.9812 & 4.4313 & 4.8812\\
DeepSeek-Flash & AZ & 159/167 & 159/167 & 114.5 & 0.8758 & 0.8764 & 0.8173 & 3.8263 & 4.1976\\
DeepSeek-Flash & CO & 159/167 & 159/167 & 114.5 & 0.9233 & 0.9228 & 0.8605 & 4.0189 & 4.4088\\
GLM-5.3-Flash & AZ & 77/167 & 77/167 & 457.7 & 0.3939 & 0.3514 & 0.4096 & 1.9641 & 2.0838\\
GLM-5.3-Flash & CO & 77/167 & 77/167 & 457.7 & 0.9353 & 0.8922 & 0.9148 & 4.2597 & 4.5195\\
Codex-GPT & AZ & 166/167 & 166/167 & 219.5 & 0.9485 & 0.9189 & 0.9759 & 4.5389 & 4.7964\\
Codex-GPT & CO & 166/167 & 166/167 & 219.5 & 0.9543 & 0.9225 & 0.9818 & 4.5663 & 4.8253\\
Codex-DeepSeek & AZ & 149/167 & 164/167 & 1059.6 & 0.9242 & 0.8958 & 0.9699 & 4.5449 & 4.7605\\
Codex-DeepSeek & CO & 149/167 & 164/167 & 1059.6 & 0.9414 & 0.9170 & 0.9898 & 4.6280 & 4.8476\\
Codex-GLM & AZ & 131/167 & 164/167 & 394.7 & 0.8848 & 0.7876 & 0.8775 & 3.8263 & 4.0000\\
Codex-GLM & CO & 131/167 & 164/167 & 394.7 & 0.9012 & 0.7969 & 0.8955 & 3.8963 & 4.0732\\
CC-DeepSeek & AZ & 125/167 & 165/167 & 1164.7 & 0.9030 & 0.8610 & 0.9739 & 4.4910 & 4.6766\\
CC-DeepSeek & CO & 125/167 & 165/167 & 1164.7 & 0.9198 & 0.8745 & 0.9878 & 4.5455 & 4.7333\\
CC-GLM & AZ & 0/12 & 1/12 & 600.1 & 0.0435 & 0.0000 & 0.0769 & 0.4167 & 0.4167\\
CC-GLM & CO & 0/12 & 1/12 & 600.1 & 1.0000 & 0.0000 & 1.0000 & 5.0000 & 5.0000\\
\end{longtable}\endgroup


==> tables/result_domain_Process_and_Workflow_Diagrams.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：流程与工作流。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-5}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 229/229 & 229/229 & 56.9 & 0.7205 & 0.6323 & 0.8976 & 4.2402 & 3.9694\\
GPT-Image-2 & CO & 229/229 & 229/229 & 56.9 & 0.7205 & 0.6323 & 0.8976 & 4.2402 & 3.9694\\
Seedream-5.0-Pro & AZ & 136/229 & 136/229 & 50.1 & 0.4782 & 0.4429 & 0.5795 & 2.6419 & 2.5764\\
Seedream-5.0-Pro & CO & 136/229 & 136/229 & 50.1 & 0.7849 & 0.7035 & 0.9677 & 4.4485 & 4.3382\\
GPT-5.6-Sol & AZ & 225/229 & 225/229 & 120.8 & 0.8035 & 0.7242 & 0.8907 & 3.8515 & 3.9738\\
GPT-5.6-Sol & CO & 225/229 & 225/229 & 120.8 & 0.8270 & 0.7471 & 0.9109 & 3.9200 & 4.0444\\
DeepSeek-Flash & AZ & 221/229 & 221/229 & 93.2 & 0.7707 & 0.7103 & 0.8147 & 3.7467 & 3.6638\\
DeepSeek-Flash & CO & 221/229 & 221/229 & 93.2 & 0.7950 & 0.7328 & 0.8438 & 3.8824 & 3.7964\\
GLM-5.3-Flash & AZ & 101/229 & 101/229 & 429.4 & 0.3668 & 0.3287 & 0.3942 & 1.8472 & 1.9389\\
GLM-5.3-Flash & CO & 101/229 & 101/229 & 429.4 & 0.8317 & 0.7613 & 0.9105 & 4.1881 & 4.3960\\
Codex-GPT & AZ & 203/229 & 226/229 & 384.6 & 0.8122 & 0.7744 & 0.9129 & 4.0961 & 4.1747\\
Codex-GPT & CO & 203/229 & 226/229 & 384.6 & 0.8267 & 0.7898 & 0.9257 & 4.1504 & 4.2301\\
Codex-DeepSeek & AZ & 138/229 & 166/229 & 1366.5 & 0.5546 & 0.5571 & 0.6791 & 3.1397 & 3.0699\\
Codex-DeepSeek & CO & 138/229 & 166/229 & 1366.5 & 0.7405 & 0.7194 & 0.9370 & 4.3313 & 4.2349\\
Codex-GLM & AZ & 110/229 & 195/229 & 469.2 & 0.6659 & 0.6323 & 0.7483 & 3.2620 & 3.4323\\
Codex-GLM & CO & 110/229 & 195/229 & 469.2 & 0.7741 & 0.7394 & 0.8726 & 3.8308 & 4.0308\\
CC-DeepSeek & AZ & 148/229 & 179/229 & 1380.2 & 0.6070 & 0.6045 & 0.7400 & 3.4279 & 3.3755\\
CC-DeepSeek & CO & 148/229 & 179/229 & 1380.2 & 0.7433 & 0.7306 & 0.9321 & 4.3855 & 4.3184\\
CC-GLM & AZ & 0/12 & 2/12 & 600.1 & 0.0769 & 0.0909 & 0.1081 & 0.6667 & 0.8333\\
CC-GLM & CO & 0/12 & 2/12 & 600.1 & 0.6667 & 1.0000 & 0.6667 & 4.0000 & 5.0000\\
\end{longtable}\endgroup


==> tables/result_domain_Scientific_Document_Pages.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：科研文档。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-6}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 139/139 & 139/139 & 59.3 & 0.7239 & 0.5152 & 0.9208 & 4.4173 & 3.5827\\
GPT-Image-2 & CO & 139/139 & 139/139 & 59.3 & 0.7239 & 0.5152 & 0.9208 & 4.4173 & 3.5827\\
Seedream-5.0-Pro & AZ & 139/139 & 139/139 & 90.6 & 0.7475 & 0.6710 & 0.9389 & 4.3309 & 3.9568\\
Seedream-5.0-Pro & CO & 139/139 & 139/139 & 90.6 & 0.7475 & 0.6710 & 0.9389 & 4.3309 & 3.9568\\
GPT-5.6-Sol & AZ & 139/139 & 139/139 & 111.4 & 0.7845 & 0.6623 & 0.9796 & 4.3453 & 4.0432\\
GPT-5.6-Sol & CO & 139/139 & 139/139 & 111.4 & 0.7845 & 0.6623 & 0.9796 & 4.3453 & 4.0432\\
DeepSeek-Flash & AZ & 138/139 & 138/139 & 121.5 & 0.7811 & 0.6494 & 0.9118 & 4.5036 & 3.9784\\
DeepSeek-Flash & CO & 138/139 & 138/139 & 121.5 & 0.7891 & 0.6579 & 0.9180 & 4.5362 & 4.0072\\
GLM-5.3-Flash & AZ & 90/139 & 90/139 & 419.3 & 0.5152 & 0.4156 & 0.6063 & 2.9856 & 2.6403\\
GLM-5.3-Flash & CO & 90/139 & 90/139 & 419.3 & 0.8182 & 0.6857 & 0.9606 & 4.6111 & 4.0778\\
Codex-GPT & AZ & 138/139 & 139/139 & 296.6 & 0.8114 & 0.6883 & 0.9864 & 4.5612 & 4.0432\\
Codex-GPT & CO & 138/139 & 139/139 & 296.6 & 0.8114 & 0.6883 & 0.9864 & 4.5612 & 4.0432\\
Codex-DeepSeek & AZ & 86/139 & 133/139 & 1448.2 & 0.7441 & 0.5628 & 0.9412 & 4.3381 & 3.8273\\
Codex-DeepSeek & CO & 86/139 & 133/139 & 1448.2 & 0.7865 & 0.6019 & 0.9835 & 4.5338 & 4.0000\\
Codex-GLM & AZ & 86/139 & 133/139 & 452.2 & 0.7475 & 0.5844 & 0.8982 & 3.8489 & 3.6115\\
Codex-GLM & CO & 86/139 & 133/139 & 452.2 & 0.7762 & 0.6027 & 0.9341 & 4.0226 & 3.7744\\
CC-DeepSeek & AZ & 92/139 & 132/139 & 1414.8 & 0.7441 & 0.6017 & 0.9208 & 4.3381 & 3.8777\\
CC-DeepSeek & CO & 92/139 & 132/139 & 1414.8 & 0.7809 & 0.6261 & 0.9714 & 4.5682 & 4.0833\\
CC-GLM & AZ & 0/12 & 2/12 & 600.1 & 0.0370 & 0.0476 & 0.1667 & 0.5833 & 0.5833\\
CC-GLM & CO & 0/12 & 2/12 & 600.1 & 0.2500 & 0.3333 & 1.0000 & 3.5000 & 3.5000\\
\end{longtable}\endgroup


==> tables/result_domain_Scientific_Statistical_Plots.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：科研统计图。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-7}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 151/151 & 151/151 & 55.6 & 0.8146 & 0.5021 & 0.9489 & 4.2583 & 3.4503\\
GPT-Image-2 & CO & 151/151 & 151/151 & 55.6 & 0.8146 & 0.5021 & 0.9489 & 4.2583 & 3.4503\\
Seedream-5.0-Pro & AZ & 151/151 & 151/151 & 83.6 & 0.8609 & 0.6485 & 0.9660 & 4.2914 & 3.9073\\
Seedream-5.0-Pro & CO & 151/151 & 151/151 & 83.6 & 0.8609 & 0.6485 & 0.9660 & 4.2914 & 3.9073\\
GPT-5.6-Sol & AZ & 150/151 & 150/151 & 94.1 & 0.9040 & 0.7364 & 0.9809 & 4.0464 & 4.3113\\
GPT-5.6-Sol & CO & 150/151 & 150/151 & 94.1 & 0.9130 & 0.7489 & 0.9872 & 4.0733 & 4.3400\\
DeepSeek-Flash & AZ & 150/151 & 150/151 & 89.2 & 0.9106 & 0.7280 & 0.9277 & 3.8609 & 4.0662\\
DeepSeek-Flash & CO & 150/151 & 150/151 & 89.2 & 0.9136 & 0.7280 & 0.9336 & 3.8867 & 4.0933\\
GLM-5.3-Flash & AZ & 76/151 & 76/151 & 478.4 & 0.4570 & 0.3473 & 0.4872 & 2.0861 & 2.0927\\
GLM-5.3-Flash & CO & 76/151 & 76/151 & 478.4 & 0.9452 & 0.7094 & 0.9622 & 4.1447 & 4.1579\\
Codex-GPT & AZ & 150/151 & 151/151 & 286.8 & 0.9238 & 0.7364 & 0.9915 & 4.4040 & 4.3642\\
Codex-GPT & CO & 150/151 & 151/151 & 286.8 & 0.9238 & 0.7364 & 0.9915 & 4.4040 & 4.3642\\
Codex-DeepSeek & AZ & 142/151 & 151/151 & 917.1 & 0.9139 & 0.7657 & 0.9702 & 4.5166 & 4.3377\\
Codex-DeepSeek & CO & 142/151 & 151/151 & 917.1 & 0.9139 & 0.7657 & 0.9702 & 4.5166 & 4.3377\\
Codex-GLM & AZ & 94/151 & 145/151 & 447.0 & 0.8344 & 0.6820 & 0.8766 & 3.4437 & 3.7616\\
Codex-GLM & CO & 94/151 & 145/151 & 447.0 & 0.8750 & 0.7118 & 0.9196 & 3.5862 & 3.9172\\
CC-DeepSeek & AZ & 129/151 & 151/151 & 990.1 & 0.9040 & 0.7448 & 0.9915 & 4.5894 & 4.3444\\
CC-DeepSeek & CO & 129/151 & 151/151 & 990.1 & 0.9040 & 0.7448 & 0.9915 & 4.5894 & 4.3444\\
CC-GLM & AZ & 0/12 & 3/12 & 600.1 & 0.2000 & 0.2000 & 0.2308 & 1.0833 & 1.0833\\
CC-GLM & CO & 0/12 & 3/12 & 600.1 & 1.0000 & 1.0000 & 1.0000 & 4.3333 & 4.3333\\
\end{longtable}\endgroup


==> tables/result_domain_System_and_Architecture_Diagrams.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{领域分组：系统与架构。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-domain-8}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 134/134 & 134/134 & 52.0 & 0.7977 & 0.6277 & 0.8204 & 4.2463 & 4.2463\\
GPT-Image-2 & CO & 134/134 & 134/134 & 52.0 & 0.7977 & 0.6277 & 0.8204 & 4.2463 & 4.2463\\
Seedream-5.0-Pro & AZ & 134/134 & 134/134 & 79.9 & 0.8132 & 0.6596 & 0.9598 & 4.3731 & 4.4701\\
Seedream-5.0-Pro & CO & 134/134 & 134/134 & 79.9 & 0.8132 & 0.6596 & 0.9598 & 4.3731 & 4.4701\\
GPT-5.6-Sol & AZ & 118/134 & 118/134 & 96.8 & 0.7860 & 0.6543 & 0.7185 & 2.4478 & 3.7612\\
GPT-5.6-Sol & CO & 118/134 & 118/134 & 96.8 & 0.8821 & 0.7235 & 0.8196 & 2.7797 & 4.2712\\
DeepSeek-Flash & AZ & 115/134 & 115/134 & 170.4 & 0.7393 & 0.6117 & 0.7158 & 3.2388 & 3.6567\\
DeepSeek-Flash & CO & 115/134 & 115/134 & 170.4 & 0.8920 & 0.7566 & 0.8423 & 3.7739 & 4.2609\\
GLM-5.3-Flash & AZ & 32/134 & 32/134 & 536.8 & 0.1790 & 0.1649 & 0.2011 & 0.8806 & 1.0597\\
GLM-5.3-Flash & CO & 32/134 & 32/134 & 536.8 & 0.8214 & 0.7561 & 0.8523 & 3.6875 & 4.4375\\
Codex-GPT & AZ & 132/134 & 133/134 & 269.5 & 0.8716 & 0.7340 & 0.9035 & 3.8060 & 4.5075\\
Codex-GPT & CO & 132/134 & 133/134 & 269.5 & 0.8750 & 0.7340 & 0.9084 & 3.8346 & 4.5414\\
Codex-DeepSeek & AZ & 90/134 & 117/134 & 1244.8 & 0.7276 & 0.6011 & 0.7855 & 3.7239 & 3.9104\\
Codex-DeepSeek & CO & 90/134 & 117/134 & 1244.8 & 0.8274 & 0.6890 & 0.9128 & 4.2650 & 4.4786\\
Codex-GLM & AZ & 78/134 & 128/134 & 460.3 & 0.8016 & 0.7021 & 0.7936 & 3.3507 & 3.9552\\
Codex-GLM & CO & 78/134 & 128/134 & 460.3 & 0.8306 & 0.7253 & 0.8245 & 3.5078 & 4.1406\\
CC-DeepSeek & AZ & 83/134 & 117/134 & 1368.6 & 0.6848 & 0.5638 & 0.7748 & 3.5896 & 3.7910\\
CC-DeepSeek & CO & 83/134 & 117/134 & 1368.6 & 0.8000 & 0.6752 & 0.8975 & 4.1111 & 4.3419\\
CC-GLM & AZ & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
CC-GLM & CO & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
\end{longtable}\endgroup


==> tables/result_rendering_mode_graphviz_dot.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{渲染模式分组：DOT。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-rendering_mode-0}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 229/229 & 229/229 & 56.9 & 0.7205 & 0.6323 & 0.8976 & 4.2402 & 3.9694\\
GPT-Image-2 & CO & 229/229 & 229/229 & 56.9 & 0.7205 & 0.6323 & 0.8976 & 4.2402 & 3.9694\\
Seedream-5.0-Pro & AZ & 136/229 & 136/229 & 50.1 & 0.4782 & 0.4429 & 0.5795 & 2.6419 & 2.5764\\
Seedream-5.0-Pro & CO & 136/229 & 136/229 & 50.1 & 0.7849 & 0.7035 & 0.9677 & 4.4485 & 4.3382\\
GPT-5.6-Sol & AZ & 225/229 & 225/229 & 120.8 & 0.8035 & 0.7242 & 0.8907 & 3.8515 & 3.9738\\
GPT-5.6-Sol & CO & 225/229 & 225/229 & 120.8 & 0.8270 & 0.7471 & 0.9109 & 3.9200 & 4.0444\\
DeepSeek-Flash & AZ & 221/229 & 221/229 & 93.2 & 0.7707 & 0.7103 & 0.8147 & 3.7467 & 3.6638\\
DeepSeek-Flash & CO & 221/229 & 221/229 & 93.2 & 0.7950 & 0.7328 & 0.8438 & 3.8824 & 3.7964\\
GLM-5.3-Flash & AZ & 101/229 & 101/229 & 429.4 & 0.3668 & 0.3287 & 0.3942 & 1.8472 & 1.9389\\
GLM-5.3-Flash & CO & 101/229 & 101/229 & 429.4 & 0.8317 & 0.7613 & 0.9105 & 4.1881 & 4.3960\\
Codex-GPT & AZ & 203/229 & 226/229 & 384.6 & 0.8122 & 0.7744 & 0.9129 & 4.0961 & 4.1747\\
Codex-GPT & CO & 203/229 & 226/229 & 384.6 & 0.8267 & 0.7898 & 0.9257 & 4.1504 & 4.2301\\
Codex-DeepSeek & AZ & 138/229 & 166/229 & 1366.5 & 0.5546 & 0.5571 & 0.6791 & 3.1397 & 3.0699\\
Codex-DeepSeek & CO & 138/229 & 166/229 & 1366.5 & 0.7405 & 0.7194 & 0.9370 & 4.3313 & 4.2349\\
Codex-GLM & AZ & 110/229 & 195/229 & 469.2 & 0.6659 & 0.6323 & 0.7483 & 3.2620 & 3.4323\\
Codex-GLM & CO & 110/229 & 195/229 & 469.2 & 0.7741 & 0.7394 & 0.8726 & 3.8308 & 4.0308\\
CC-DeepSeek & AZ & 148/229 & 179/229 & 1380.2 & 0.6070 & 0.6045 & 0.7400 & 3.4279 & 3.3755\\
CC-DeepSeek & CO & 148/229 & 179/229 & 1380.2 & 0.7433 & 0.7306 & 0.9321 & 4.3855 & 4.3184\\
CC-GLM & AZ & 0/12 & 2/12 & 600.1 & 0.0769 & 0.0909 & 0.1081 & 0.6667 & 0.8333\\
CC-GLM & CO & 0/12 & 2/12 & 600.1 & 0.6667 & 1.0000 & 0.6667 & 4.0000 & 5.0000\\
\end{longtable}\endgroup


==> tables/result_rendering_mode_html_browser.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{渲染模式分组：HTML。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-rendering_mode-1}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 526/526 & 526/526 & 55.8 & 0.7031 & 0.4136 & 0.9444 & 4.6527 & 3.5802\\
GPT-Image-2 & CO & 526/526 & 526/526 & 55.8 & 0.7031 & 0.4136 & 0.9444 & 4.6527 & 3.5802\\
Seedream-5.0-Pro & AZ & 526/526 & 526/526 & 88.6 & 0.7926 & 0.6044 & 0.9478 & 4.5951 & 3.9259\\
Seedream-5.0-Pro & CO & 526/526 & 526/526 & 88.6 & 0.7926 & 0.6044 & 0.9478 & 4.5951 & 3.9259\\
GPT-5.6-Sol & AZ & 526/526 & 526/526 & 114.9 & 0.7681 & 0.5220 & 0.9789 & 4.5437 & 3.9658\\
GPT-5.6-Sol & CO & 526/526 & 526/526 & 114.9 & 0.7681 & 0.5220 & 0.9789 & 4.5437 & 3.9658\\
DeepSeek-Flash & AZ & 523/526 & 523/526 & 107.7 & 0.7717 & 0.5186 & 0.9254 & 4.6711 & 3.9430\\
DeepSeek-Flash & CO & 523/526 & 523/526 & 107.7 & 0.7774 & 0.5240 & 0.9312 & 4.6979 & 3.9656\\
GLM-5.3-Flash & AZ & 401/526 & 401/526 & 379.8 & 0.5996 & 0.4049 & 0.7027 & 3.6065 & 3.1483\\
GLM-5.3-Flash & CO & 401/526 & 401/526 & 379.8 & 0.8244 & 0.5675 & 0.9432 & 4.7307 & 4.1297\\
Codex-GPT & AZ & 521/526 & 526/526 & 289.8 & 0.7681 & 0.5441 & 0.9851 & 4.6977 & 4.0133\\
Codex-GPT & CO & 521/526 & 526/526 & 289.8 & 0.7681 & 0.5441 & 0.9851 & 4.6977 & 4.0133\\
Codex-DeepSeek & AZ & 455/526 & 517/526 & 1122.7 & 0.7446 & 0.4988 & 0.9677 & 4.6369 & 3.9259\\
Codex-DeepSeek & CO & 455/526 & 517/526 & 1122.7 & 0.7590 & 0.5083 & 0.9848 & 4.7176 & 3.9942\\
Codex-GLM & AZ & 374/526 & 518/526 & 425.1 & 0.7726 & 0.5371 & 0.9279 & 4.1844 & 3.7985\\
Codex-GLM & CO & 374/526 & 518/526 & 425.1 & 0.7826 & 0.5415 & 0.9407 & 4.2490 & 3.8571\\
CC-DeepSeek & AZ & 465/526 & 519/526 & 1052.0 & 0.7572 & 0.5186 & 0.9658 & 4.6635 & 3.9563\\
CC-DeepSeek & CO & 465/526 & 519/526 & 1052.0 & 0.7670 & 0.5240 & 0.9798 & 4.7264 & 4.0096\\
CC-GLM & AZ & 0/36 & 12/36 & 600.1 & 0.1392 & 0.1231 & 0.3302 & 1.5556 & 1.2222\\
CC-GLM & CO & 0/36 & 12/36 & 600.1 & 0.4074 & 0.3636 & 0.9722 & 4.6667 & 3.6667\\
\end{longtable}\endgroup


==> tables/result_rendering_mode_latex_circuitikz.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{渲染模式分组：CircuitikZ。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-rendering_mode-2}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 161/161 & 161/161 & 44.4 & 0.7203 & 0.6592 & 0.9516 & 4.3851 & 3.9752\\
GPT-Image-2 & CO & 161/161 & 161/161 & 44.4 & 0.7203 & 0.6592 & 0.9516 & 4.3851 & 3.9752\\
Seedream-5.0-Pro & AZ & 161/161 & 161/161 & 72.5 & 0.7814 & 0.7309 & 0.9626 & 4.4348 & 4.0621\\
Seedream-5.0-Pro & CO & 161/161 & 161/161 & 72.5 & 0.7814 & 0.7309 & 0.9626 & 4.4348 & 4.0621\\
GPT-5.6-Sol & AZ & 146/161 & 146/161 & 73.7 & 0.6945 & 0.6592 & 0.8374 & 3.1056 & 3.6894\\
GPT-5.6-Sol & CO & 146/161 & 146/161 & 73.7 & 0.7742 & 0.7424 & 0.9270 & 3.4247 & 4.0685\\
DeepSeek-Flash & AZ & 136/161 & 136/161 & 181.9 & 0.6495 & 0.5605 & 0.7429 & 3.4099 & 3.2795\\
DeepSeek-Flash & CO & 136/161 & 136/161 & 181.9 & 0.7860 & 0.6983 & 0.8942 & 4.0368 & 3.8824\\
GLM-5.3-Flash & AZ & 29/161 & 29/161 & 548.3 & 0.1415 & 0.1211 & 0.1604 & 0.8137 & 0.7578\\
GLM-5.3-Flash & CO & 29/161 & 29/161 & 548.3 & 0.8148 & 0.7297 & 0.9605 & 4.5172 & 4.2069\\
Codex-GPT & AZ & 153/161 & 154/161 & 200.8 & 0.7814 & 0.7713 & 0.9253 & 4.1180 & 4.1429\\
Codex-GPT & CO & 153/161 & 154/161 & 200.8 & 0.8046 & 0.7854 & 0.9590 & 4.3052 & 4.3312\\
Codex-DeepSeek & AZ & 141/161 & 152/161 & 950.2 & 0.7267 & 0.6861 & 0.9055 & 4.1677 & 4.1056\\
Codex-DeepSeek & CO & 141/161 & 152/161 & 950.2 & 0.7740 & 0.7251 & 0.9581 & 4.4145 & 4.3487\\
Codex-GLM & AZ & 107/161 & 157/161 & 430.3 & 0.7042 & 0.6816 & 0.8725 & 3.4037 & 3.5839\\
Codex-GLM & CO & 107/161 & 157/161 & 430.3 & 0.7180 & 0.6972 & 0.8941 & 3.4904 & 3.6752\\
CC-DeepSeek & AZ & 129/161 & 146/161 & 1083.3 & 0.7203 & 0.6682 & 0.8769 & 3.9068 & 3.7081\\
CC-DeepSeek & CO & 129/161 & 146/161 & 1083.3 & 0.7860 & 0.7198 & 0.9614 & 4.3082 & 4.0890\\
CC-GLM & AZ & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
CC-GLM & CO & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
\end{longtable}\endgroup


==> tables/result_rendering_mode_latex_tikz.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{渲染模式分组：TikZ。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-rendering_mode-3}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 134/134 & 134/134 & 52.0 & 0.7977 & 0.6277 & 0.8204 & 4.2463 & 4.2463\\
GPT-Image-2 & CO & 134/134 & 134/134 & 52.0 & 0.7977 & 0.6277 & 0.8204 & 4.2463 & 4.2463\\
Seedream-5.0-Pro & AZ & 134/134 & 134/134 & 79.9 & 0.8132 & 0.6596 & 0.9598 & 4.3731 & 4.4701\\
Seedream-5.0-Pro & CO & 134/134 & 134/134 & 79.9 & 0.8132 & 0.6596 & 0.9598 & 4.3731 & 4.4701\\
GPT-5.6-Sol & AZ & 118/134 & 118/134 & 96.8 & 0.7860 & 0.6543 & 0.7185 & 2.4478 & 3.7612\\
GPT-5.6-Sol & CO & 118/134 & 118/134 & 96.8 & 0.8821 & 0.7235 & 0.8196 & 2.7797 & 4.2712\\
DeepSeek-Flash & AZ & 115/134 & 115/134 & 170.4 & 0.7393 & 0.6117 & 0.7158 & 3.2388 & 3.6567\\
DeepSeek-Flash & CO & 115/134 & 115/134 & 170.4 & 0.8920 & 0.7566 & 0.8423 & 3.7739 & 4.2609\\
GLM-5.3-Flash & AZ & 32/134 & 32/134 & 536.8 & 0.1790 & 0.1649 & 0.2011 & 0.8806 & 1.0597\\
GLM-5.3-Flash & CO & 32/134 & 32/134 & 536.8 & 0.8214 & 0.7561 & 0.8523 & 3.6875 & 4.4375\\
Codex-GPT & AZ & 132/134 & 133/134 & 269.5 & 0.8716 & 0.7340 & 0.9035 & 3.8060 & 4.5075\\
Codex-GPT & CO & 132/134 & 133/134 & 269.5 & 0.8750 & 0.7340 & 0.9084 & 3.8346 & 4.5414\\
Codex-DeepSeek & AZ & 90/134 & 117/134 & 1244.8 & 0.7276 & 0.6011 & 0.7855 & 3.7239 & 3.9104\\
Codex-DeepSeek & CO & 90/134 & 117/134 & 1244.8 & 0.8274 & 0.6890 & 0.9128 & 4.2650 & 4.4786\\
Codex-GLM & AZ & 78/134 & 128/134 & 460.3 & 0.8016 & 0.7021 & 0.7936 & 3.3507 & 3.9552\\
Codex-GLM & CO & 78/134 & 128/134 & 460.3 & 0.8306 & 0.7253 & 0.8245 & 3.5078 & 4.1406\\
CC-DeepSeek & AZ & 83/134 & 117/134 & 1368.6 & 0.6848 & 0.5638 & 0.7748 & 3.5896 & 3.7910\\
CC-DeepSeek & CO & 83/134 & 117/134 & 1368.6 & 0.8000 & 0.6752 & 0.8975 & 4.1111 & 4.3419\\
CC-GLM & AZ & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
CC-GLM & CO & 0/12 & 0/12 & 600.1 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\
\end{longtable}\endgroup


==> tables/result_rendering_mode_python_cli.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{llrrr rrrrr}
\caption{渲染模式分组：Python。AZ 为失败计零，CO 为成功评分；两者均纳入恢复产物。}\label{tab:app-rendering_mode-4}\\
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endfirsthead
\toprule
方法 & 集合 & 正常 & 含恢复 & 秒 & Dir. & Der. & Inv. & VQ & DQ\\\midrule
\endhead
\bottomrule\endfoot
GPT-Image-2 & AZ & 523/523 & 523/523 & 46.6 & 0.7490 & 0.5395 & 0.9084 & 4.4665 & 3.7457\\
GPT-Image-2 & CO & 523/523 & 523/523 & 46.6 & 0.7490 & 0.5395 & 0.9084 & 4.4665 & 3.7457\\
Seedream-5.0-Pro & AZ & 521/523 & 521/523 & 73.4 & 0.8193 & 0.6837 & 0.9338 & 4.3614 & 3.9790\\
Seedream-5.0-Pro & CO & 521/523 & 521/523 & 73.4 & 0.8258 & 0.6907 & 0.9384 & 4.3781 & 3.9942\\
GPT-5.6-Sol & AZ & 514/523 & 514/523 & 84.9 & 0.8877 & 0.7946 & 0.9579 & 4.3614 & 4.4971\\
GPT-5.6-Sol & CO & 514/523 & 514/523 & 84.9 & 0.9063 & 0.8091 & 0.9736 & 4.4377 & 4.5759\\
DeepSeek-Flash & AZ & 494/523 & 494/523 & 107.2 & 0.8359 & 0.7436 & 0.7822 & 3.7744 & 3.9312\\
DeepSeek-Flash & CO & 494/523 & 494/523 & 107.2 & 0.8898 & 0.7868 & 0.8299 & 3.9960 & 4.1619\\
GLM-5.3-Flash & AZ & 230/523 & 230/523 & 479.0 & 0.3789 & 0.3240 & 0.3849 & 1.8298 & 1.8834\\
GLM-5.3-Flash & CO & 230/523 & 230/523 & 479.0 & 0.9087 & 0.7791 & 0.8860 & 4.1609 & 4.2826\\
Codex-GPT & AZ & 516/523 & 517/523 & 221.9 & 0.8926 & 0.8036 & 0.9703 & 4.5660 & 4.5793\\
Codex-GPT & CO & 516/523 & 517/523 & 221.9 & 0.9014 & 0.8098 & 0.9818 & 4.6190 & 4.6325\\
Codex-DeepSeek & AZ & 475/523 & 515/523 & 917.1 & 0.8838 & 0.7972 & 0.9585 & 4.5755 & 4.5430\\
Codex-DeepSeek & CO & 475/523 & 515/523 & 917.1 & 0.8943 & 0.8054 & 0.9736 & 4.6466 & 4.6136\\
Codex-GLM & AZ & 363/523 & 495/523 & 427.1 & 0.8242 & 0.7117 & 0.8397 & 3.7725 & 3.8509\\
Codex-GLM & CO & 363/523 & 495/523 & 427.1 & 0.8683 & 0.7391 & 0.8869 & 3.9859 & 4.0687\\
CC-DeepSeek & AZ & 440/523 & 518/523 & 968.9 & 0.8799 & 0.7832 & 0.9759 & 4.6157 & 4.5010\\
CC-DeepSeek & CO & 440/523 & 518/523 & 968.9 & 0.8886 & 0.7902 & 0.9862 & 4.6602 & 4.5444\\
CC-GLM & AZ & 5/36 & 10/36 & 580.2 & 0.1857 & 0.1091 & 0.2478 & 1.3056 & 1.2222\\
CC-GLM & CO & 5/36 & 10/36 & 580.2 & 0.9286 & 0.7500 & 1.0000 & 4.7000 & 4.4000\\
\end{longtable}\endgroup


==> tables/results_difficulty.tex <==
\input{tables/result_difficulty_easy.tex}
\input{tables/result_difficulty_middle.tex}
\input{tables/result_difficulty_hard.tex}

==> tables/results_domain.tex <==
\input{tables/result_domain_Business_Web_Interfaces.tex}
\input{tables/result_domain_Chemistry_and_Molecular_Figures.tex}
\input{tables/result_domain_Circuit_and_Logic_Diagrams.tex}
\input{tables/result_domain_Interactive_Data_Panels.tex}
\input{tables/result_domain_Mathematical_and_Geometric_Figures.tex}
\input{tables/result_domain_Process_and_Workflow_Diagrams.tex}
\input{tables/result_domain_Scientific_Document_Pages.tex}
\input{tables/result_domain_Scientific_Statistical_Plots.tex}
\input{tables/result_domain_System_and_Architecture_Diagrams.tex}

==> tables/results_rendering_mode.tex <==
\input{tables/result_rendering_mode_graphviz_dot.tex}
\input{tables/result_rendering_mode_html_browser.tex}
\input{tables/result_rendering_mode_latex_circuitikz.tex}
\input{tables/result_rendering_mode_latex_tikz.tex}
\input{tables/result_rendering_mode_python_cli.tex}
